E3: Ensemble of Expert Embedders for Adapting Synthetic Image Detectors to New Generators Using Limited Data

As generative AI progresses rapidly, new synthetic image generators continue to emerge at a swift pace. Traditional detection methods face two main challenges in adapting to these generators: the forensic traces of synthetic images from new techniques can vastly differ from those learned during training, and access to data for these new generators is often limited. To address these issues, we introduce the Ensemble of Expert Embedders (E3), a novel continual learning framework for updating synthetic image detectors. E3 enables the accurate detection of images from newly emerged generators using minimal training data. Our approach does this by first employing transfer learning to develop a suite of expert embedders, each specializing in the forensic traces of a specific generator. Then, all embeddings are jointly analyzed by an Expert Knowledge Fusion Network to produce accurate and reliable detection decisions. Our experiments demonstrate that E3 outperforms existing continual learning methods, including those developed specifically for synthetic image detection.

==> figures/expert_knowledge_fusion_v0-.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/expert_knowledge_fusion_v1.png}
    \pulluppp
    \caption{The architecture of our Expert Knowledge Fusion Network (EKFN). All experts $\{\phi_0, ..., \phi_k\}$ are frozen during the training phase of the EKFN. As new experts emerge, the EKFN is reinitialized with the appropriate input size and retrained using the memory $\mathcal{M}_k$.}
    \label{fig:expert_knowledge_fusion_net}
    \pulluppp
\end{figure}

==> figures/new_expert_training.tex <==
\begin{figure}[!t]
    \centering

    \includegraphics[width=\linewidth]{figures/new_expert_training_diagram.png}
    \pulluppp\pullupp
    \caption{When new generators appear, we introduce a new expert embedder finetuned from the base $\phi_0$ using generator $g_k$'s data $\mathcal{D}_k$. Memory $\mathcal{M}$, fixed in size, evenly splits between real and synthetic images. With more generators, $\mathcal{M}$'s synthetic segment is evenly divided to ensure equal representation of each generator.}
    \label{fig:overall_sys_diagram}
    \pulluppp
\end{figure}


==> figures/overall_training_procedure_v0.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{figures/Training-Procedure-All-.png}
\pulluppp\pullupp
\caption{On the \textit{left}, the training process for a new expert embedder is illustrated. Upon the emergence of a new generator $g_k$, a new expert embedder $\phi_k$ is created by finetuning the base embedder $\phi_0$ with synthetic images $\mathcal{D}_k$ from $g_k$ and real images $\mathcal{R}$ from memory $\mathcal{M}$. After its creation, $\phi_k$'s weights are permanently frozen. The \textit{right} side demonstrates the update process for the Expert Knowledge Fusion Network (EKFN) following the introduction of a new expert embedder. Images from $\mathcal{M}$ are processed through all experts, and the resulting embeddings are passed into a transformer and subsequently an MLP layer. The MLP's decision is used to calculate a Binary Cross Entropy Loss, facilitating the update of EKFN's components.  The training procedure is detailed further in Sec.~\ref{sec:proposed_approach}.}

% I have not removed the portion where I talk about how memory is managed, the figure detail was too long.

% \caption{This figure outlines our method's training process to update its components. On the left, the process of training a new expert embedder is depicted. When a new generator $g_k$ appears, we create a new expert embedder $\phi_k$ by finetuning the base embedder $\phi_0$ with synthetic images $\mathcal{D}_k$ from $g_k$ and real images $\mathcal{R}$ from the memory $\mathcal{M}$. Once created, $\phi_k$'s weights are frozen. The memory buffer $\mathcal{M}$, fixed in size, is divided evenly between real and synthetic images, adjusting for equal representation as more generators emerge. The right side shows how Expert Knowledge Fusion Network (EKFN) is updated when a new generator is introduced. Images from $\mathcal{M}$ are processed through all frozen expert embedders, with the embeddings fed into a transformer and then an MLP layer. The MLP's output calculates a Binary Cross Entropy Loss to update EKFN's components. The training procedure is detailed further in Sec.~\ref{sec:proposed_approach}.}
\label{fig:overall_sys_diagram}
\end{figure*}

==> sec/EKFN_v0.tex <==


\input{figures/expert_knowledge_fusion_v0}


\subsection{Training Expert Knowledge Fusion Network}
After training the expert embedder $\phi_k$, we train the EKFN, which we refer to as $\psi$ to have a uniform notation to perform classification. The only training data used in this step is a new version of $\mathcal{M}$ updated with the recently observed synthetic images, $\mathcal{D}_k$.
This network needs to make a decision based on the sequence of embeddings, $\mathcal{L}$, produced by the set of existing embedders, $\mathcal{E} = \{ \phi_1, \ldots, \phi_k  \}$ for each image in $\mathcal{M}$.

%, which we define as $\mathcal{L}_k = \{\ubar{x}{l} \: | \: \varphi_l \in \{ \phi_1, \ldots, \phi_k  \} \}$.
%
The network analyzes $\mathcal{L}$, using a transformer to treat each input embedding as a token in a sequence of forensic evidence. The transformer's output associated with each of the embeddings ($\ubar{x}{l}$s), which we refer to as $\ubar{z}{l}$s, contains information about the relevance of $\ubar{x}{l}$  with respect to itself and other embeddings in $\mathcal{E}$. We use EKFN to produce a vector $\ubar{z}{l}$ for each corresponding element in $\mathcal{E}$. We then scale $\mathcal{L}$ by $\ubar{z}{l}$s using the Hadamard product (element-wise product). Subsequently, we provide the sequence of scaled embeddings to a classifier network composed of only a few linear layers. The training procedure of EKFN is provided in Alg.~\ref{alg:train_ekfn}. Additionally, the network's architecture is depicted in Fig.~\ref{fig:expert_knowledge_fusion_net}.

\begin{algorithm}
	\begin{algorithmic}[1]
		\Procedure{TrainEKFN}{$\mathcal{M}, \mathcal{D}_{k},  \mathcal{E}, \mathcal{P}$}
		
		\State Update $\mathcal{M}$ with $\mathcal{D}_{k}$
		
		\For{$i \in  \mathcal{M} $}
			\State $\mathcal{L} \gets \{\ubar{x}{l} \: | \: \phi_l \in \mathcal{E} \}$
            % \State Apply $\mathcal{E}$ on $i$ to get $\mathcal{L}$ 
			\State Feed $\mathcal{L}$ to the transformer to form $\mathcal{Z}$ of $\ubar{z}{l}$s
			% \State Scale $\mathcal{L}$ by $\ubar{z}{l}$s
            \State $\mathcal{L} \gets \{  \ubar{x}{l} \odot \ubar{z}{l} | \ubar{x}{l} \in \mathcal{E}, \ubar{z}{l} \in \mathcal{Z} \}$
            \State Feed $\mathcal{L}$ to the linear layers
			\State Calculate the BCE loss
			\State Back-propagate loss to train the EKFN
		
      	\EndFor
		\EndProcedure
	\end{algorithmic}
    \caption{\:\: Training \Reasoner} \label{alg:train_ekfn}
\end{algorithm}

==> sec/EKFN_v1_Aref.tex <==


\input{figures/expert_knowledge_fusion_v0}


\subsection{Training Expert Knowledge Fusion Network}
\label{subsec:ekfn_training}

After adding the expert embedder $\phi_k$ to the set of existing \ee, we train the EKFN to perform classification. We will refer to the EKFN as $\psi$ in the following to have a uniform notation. To train $\psi$, we first need to update the memory buffer using $\mathcal{D}_k$.

\subheader{Updating Memory Buffer}
\label{subheader:mem}
To update the memory buffer to obtain $\mathcal{M}_k$, we use the same set of real data, $\mathcal{R}$, used to train $\phi_k$. However, to have a balanced representation of all known generators, we need to include a subset of $\mathcal{D}_k$ in the memory buffer. We form $\mathcal{S}_k$, the synthetic portion of $\mathcal{M}_k$, by retaining $P_k$ number of images from each generator, where $P_k$ is defined as follows:
\begin{equation}
    \small
    P_k = \floor*{\dfrac{M}{2(k+1)}}
\end{equation}

Therefore, after adding generator $g_k$, the number of synthetic images in $\mathcal{S}_k$ will be equal to $(k+1)P_k$, which is equal or close to ${M}/{2}$, as desired. Then, we construct $\mathcal{S}_k$ by pulling $P_k$ images per generator from $\mathcal{S}_{k-1}$ and $P_k$ images from $\mathcal{D}_k$. Effectively, $S_{k}$ consists of ${M}/{2}$ data points created by each generator in $\mathcal{G}_k$. Finally, we define:

\begin{equation}
    \mathcal{M}_k = \mathcal{S}_k \cup \mathcal{R}
\end{equation}



\begin{algorithm}[!t]
	\begin{algorithmic}
		\Require $\mathcal{M}_{k-1}, \mathcal{D}_{k}, \Phi_k$
		\\
        // Let $\omega_M^{(k-1)}$ be the procedure to select a subset of images from $\mathcal{M}_{k-1}$
        \\
        // Let $\omega_D^{(k)}$ be the procedure to select a subset of images from $\mathcal{D}_{k}$.
        \\
        // Let $\mathcal{Q}$ be the transformer in the network
        \\
        // Let $\mathcal{W}$ be the MLP layers after the transformer in the network
        \\
		$\mathcal{M}_k \gets \omega_M^{(k-1)}(\mathcal{M}_{k-1}) \cup \omega_D^{(k)}(\mathcal{D}_{k})$
        \Repeat
            \State $\mathcal{L}_\psi \gets 0$
    		\For {$i = 1; \;\; i \leq |\mathcal{M}_k|; \;\; i \pluseq 1$}
                \State$I_i = \mathcal{M}_k\left[i\right]$
                \State $\mathbf{X} \gets \{\empty\}$
                \For {$\ell = 1; \;\; \ell \leq |\Phi_k|; \;\; \ell \pluseq 1$}
                    \State $\phi_{\ell} \gets \Phi_k\left[\ell\right]$
                    \State $\mathbf{X} \gets \mathbf{X} \cup \{\phi_{\ell}(I_i)\}$
                \EndFor
    			\State $\mathbf{Z} \gets \mathcal{Q}(\mathbf{X})$
                \For {$j = 1; \;\; j \leq |\mathbf{Z}|; \;\; j \pluseq 1$}
                    \State $\ubar{z}{j} \gets \mathbf{Z}\left[j\right], \; \ubar{x}{j} \gets \mathbf{X}\left[j\right]$
                    \State $\ubar{z}{j} \gets \ubar{x}{j} \odot \ubar{z}{j}$ \Comment{$\odot$ is the Hadamard product}
                \EndFor
                \State $\hat{y}_i \gets \mathcal{W}(\mathbf{Z})$ % \Comment{$\hat{y}_i$ is detection score}
                \State $\mathcal{L}_\psi \gets \mathcal{L}_\psi - ( \hat{y}_i \log{(t_i)} + (1 - \hat{y}_i) \log{(1 - t_i)}) $
            \EndFor
            \State $\psi_k \gets \text{Back-propagate}(\mathcal{L}_\psi, \psi_k)$ 
        \Until {max epoch is reached}
        \\
        \Return $\psi_k$
	\end{algorithmic}
    \caption{\:\: Training \Reasoner} \label{alg:train_ekfn}
\end{algorithm}







\subheader{Training EKFN}
Now, we can use $\mathcal{M}_k$ to train $\psi$. This network needs to make a decision based on the sequence of embeddings, $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$, which is produced by $\Phi_k$ for each input image. The network analyzes this set of embeddings using a transformer to treat each input embedding as a token in a sequence of forensic evidence. The transformer's output associated with each of the embeddings, which we refer to as $\ubar{z}{\ell}$, contains information about the relevance of $\ubar{x}{\ell}$  with respect to itself and other embeddings in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$.  
We then scale $\ubar{x}{\ell}$ by $\ubar{z}{\ell}$ using the Hadamard product (element-wise product), which will be denoted as $\odot$. Subsequently, we provide the sequence of scaled embeddings to a classifier network composed of only a few linear layers. Next, using the following loss function:.
\begin{dmath}
    \label{eq:l_ekfn}
    \mathcal{L}_\psi = 
    \sum_{I_\ell \in \mathcal{M}_k} \psi(\{\ubar{x}{1}^\ell, \ldots, \ubar{x}{k}^\ell \}) \log{t_\ell} +
    (1 - \psi(\{\ubar{x}{1}^\ell, \ldots, \ubar{x}{k}^\ell \})) \log(1-t_\ell)
\end{dmath}
where $t_\ell$ is the ground-truth label for $I_\ell$, we optimize the weights of the network.

The training procedure of EKFN is provided in Alg.~\ref{alg:train_ekfn}. Additionally, the network's architecture is depicted in Fig.~\ref{fig:expert_knowledge_fusion_net}.

%, which we define as $\mathcal{L}_k = \{\ubar{x}{l} \: | \: \varphi_l \in \{ \phi_1, \ldots, \phi_k  \} \}$.

%We use $\psi$ to produce a vector $\ubar{z}{\ell}$ for each corresponding element in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$.




% \State $\mathbf{X} \gets \{   \phi_{\ell}(i) \: | \: \phi_{\ell} \in \Phi_k \}$
% \State $\mathbf{Z} \gets \{  \ubar{x}{l} \odot \ubar{z}{l} | \ubar{x}{l} \in \mathbf{X}, \ubar{z}{l} \in \mathbf{Z} \}$












==> sec/EKFN_v2_Tai.tex <==


\input{figures/expert_knowledge_fusion_v0}


\subsection{Training Expert Knowledge Fusion Network}
\label{subsec:ekfn_training}

After adding the expert embedder $\phi_k$ to the set of existing \ee, we train the Expert Knowledge Fusion Network (EKFN) to perform classification. We will refer to the EKFN as $\psi$ in the following to have a uniform notation. To train $\psi$, we first need to update the memory buffer using $\mathcal{D}_k$. In the following, we first discuss the architecture of EKFN, and then we talk how the memory buffer is updated when a new generator shows up, and finally explain the training procedure of EKFN.

\subheader{Updating Memory Buffer}
\label{subheader:mem}
To update the memory buffer to obtain $\mathcal{M}_k$, we use the same set of real data, $\mathcal{R}$, used to train $\phi_k$. However, to have a balanced representation of all known generators, we need to include a subset of $\mathcal{D}_k$ in the memory buffer. We form $\mathcal{S}_k$, the synthetic portion of $\mathcal{M}_k$, by retaining $P_k$ number of images from each generator, where $P_k$ is defined as follows:
\begin{equation}
    \small
    P_k = \floor*{\dfrac{M}{2(k+1)}}
\end{equation}

Therefore, after adding generator $g_k$, the number of synthetic images in $\mathcal{S}_k$ will be equal to $(k+1)P_k$, which is equal or close to ${M}/{2}$, as desired. Then, we construct $\mathcal{S}_k$ by pulling $P_k$ images per generator from $\mathcal{S}_{k-1}$ and $P_k$ images from $\mathcal{D}_k$. Effectively, $S_{k}$ consists of ${M}/{2}$ data points created by each generator in $\mathcal{G}_k$. Finally, we define:

\begin{equation}
    \mathcal{M}_k = \mathcal{S}_k \cup \mathcal{R}
\end{equation}



\begin{algorithm}[!t]
	\begin{algorithmic}
		\Require $\mathcal{M}_{k-1}, \mathcal{D}_{k}, \Phi_k$
		\\
        // Let $\omega_M^{(k-1)}$ be the procedure to select a subset of images from $\mathcal{M}_{k-1}$
        \\
        // Let $\omega_D^{(k)}$ be the procedure to select a subset of images from $\mathcal{D}_{k}$.
        \\
        // Let $\mathcal{Q}$ be the transformer in the network
        \\
        // Let $\mathcal{W}$ be the MLP layers after the transformer in the network
        \\
		$\mathcal{M}_k \gets \omega_M^{(k-1)}(\mathcal{M}_{k-1}) \cup \omega_D^{(k)}(\mathcal{D}_{k})$
        \Repeat
            \State $\mathcal{L}_\psi \gets 0$
    		\For {$i = 1; \;\; i \leq |\mathcal{M}_k|; \;\; i \pluseq 1$}
                \State$I_i = \mathcal{M}_k\left[i\right]$
                \State $\mathbf{X} \gets \{\empty\}$
                \For {$\ell = 1; \;\; \ell \leq |\Phi_k|; \;\; \ell \pluseq 1$}
                    \State $\phi_{\ell} \gets \Phi_k\left[\ell\right]$
                    \State $\mathbf{X} \gets \mathbf{X} \cup \{\phi_{\ell}(I_i)\}$
                \EndFor
    			\State $\mathbf{Z} \gets \mathcal{Q}(\mathbf{X})$
                \For {$j = 1; \;\; j \leq |\mathbf{Z}|; \;\; j \pluseq 1$}
                    \State $\ubar{z}{j} \gets \mathbf{Z}\left[j\right], \; \ubar{x}{j} \gets \mathbf{X}\left[j\right]$
                    \State $\ubar{z}{j} \gets \ubar{x}{j} \odot \ubar{z}{j}$ \Comment{$\odot$ is the Hadamard product}
                \EndFor
                \State $\hat{y}_i \gets \mathcal{W}(\mathbf{Z})$ % \Comment{$\hat{y}_i$ is detection score}
                \State $\mathcal{L}_\psi \gets \mathcal{L}_\psi - ( \hat{y}_i \log{(t_i)} + (1 - \hat{y}_i) \log{(1 - t_i)}) $
            \EndFor
            \State $\psi_k \gets \text{Back-propagate}(\mathcal{L}_\psi, \psi_k)$ 
        \Until {max epoch is reached}
        \\
        \Return $\psi_k$
	\end{algorithmic}
    \caption{\:\: Training \Reasoner} \label{alg:train_ekfn}
\end{algorithm}







\subheader{Training EKFN}
Now, we can use $\mathcal{M}_k$ to train $\psi$. This network needs to make a decision based on the sequence of embeddings, $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$, which is produced by $\Phi_k$ for each input image. The network analyzes this set of embeddings using a transformer to treat each input embedding as a token in a sequence of forensic evidence. The transformer's output associated with each of the embeddings, which we refer to as $\ubar{z}{\ell}$, contains information about the relevance of $\ubar{x}{\ell}$  with respect to itself and other embeddings in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$.  
We then scale $\ubar{x}{\ell}$ by $\ubar{z}{\ell}$ using the Hadamard product (element-wise product), which will be denoted as $\odot$. Subsequently, we provide the sequence of scaled embeddings to a classifier network composed of only a few linear layers. Next, using the following loss function:.
\begin{dmath}
    \label{eq:l_ekfn}
    \mathcal{L}_\psi = 
    \sum_{I_\ell \in \mathcal{M}_k} \psi(\{\ubar{x}{1}^\ell, \ldots, \ubar{x}{k}^\ell \}) \log{t_\ell} +
    (1 - \psi(\{\ubar{x}{1}^\ell, \ldots, \ubar{x}{k}^\ell \})) \log(1-t_\ell)
\end{dmath}
where $t_\ell$ is the ground-truth label for $I_\ell$, we optimize the weights of the network.

The training procedure of EKFN is provided in Alg.~\ref{alg:train_ekfn}. Additionally, the network's architecture is depicted in Fig.~\ref{fig:expert_knowledge_fusion_net}.

%, which we define as $\mathcal{L}_k = \{\ubar{x}{l} \: | \: \varphi_l \in \{ \phi_1, \ldots, \phi_k  \} \}$.

%We use $\psi$ to produce a vector $\ubar{z}{\ell}$ for each corresponding element in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$.




% \State $\mathbf{X} \gets \{   \phi_{\ell}(i) \: | \: \phi_{\ell} \in \Phi_k \}$
% \State $\mathbf{Z} \gets \{  \ubar{x}{l} \odot \ubar{z}{l} | \ubar{x}{l} \in \mathbf{X}, \ubar{z}{l} \in \mathbf{Z} \}$












==> sec/EKFN_v3_Aref.tex <==



\subsection{Training Expert Knowledge Fusion Network}
\label{subsec:ekfn_training}

After adding the expert embedder $\phi_k$ to the set of existing \ee, we train the Expert Knowledge Fusion Network (EKFN) to perform classification. This network aims to fuse the embeddings resulted from the application of all embedders in $\Phi_k$ on each input image, and subsequently, produce a final detection decision based on the joint knowledge of all embedders.
In the following, we first discuss the update procedure of the memory buffer in the face of emergence of a new generator. Then, we explain the training procedure of EKFN, and finally, we discuss the architecture we select to use as EKFN.

%In the following, we first discuss the architecture of EKFN. Then, we talk about how the memory buffer is updated when a new generator shows up, and finally explain the training procedure of EKFN.

% We will refer to the EKFN as $\psi$ in the following to have a uniform notation. To train $\psi$, we first need to update the memory buffer using $\mathcal{D}_k$. 


\subheader{Updating Memory Buffer}
%\label{subheader:mem}
To update memory buffer $\mathcal{M}_{k-1}$ to obtain $\mathcal{M}_k$, we use the same set of real data, $\mathcal{R}$, used to train $\phi_k$. However, to have a balanced representation of all known generators, we need to include a subset of $\mathcal{D}_k$ in the memory buffer. We form $\mathcal{S}_k$, the synthetic portion of $\mathcal{M}_k$, by retaining $P_k$ number of images from each generator, where $P_k$ is defined as follows:
\begin{equation}
    \small
    P_k = \floor*{\dfrac{M}{2(k+1)}}
\end{equation}
where $\floor{\cdot}$ denotes the floor function.

Therefore, after adding generator $g_k$, the number of synthetic images in $\mathcal{S}_k$ will be equal to $(k+1)P_k$, which is equal or close to ${M}/{2}$, as desired. Then, we construct $\mathcal{S}_k$ by pulling $P_k$ images per generator from $\mathcal{S}_{k-1}$ and $P_k$ images from $\mathcal{D}_k$. Effectively, $S_{k}$ consists of ${M}/{2}$ data points equally created by generators in $\mathcal{G}_k$. Finally, we define:

\begin{equation}
    \mathcal{M}_k = \mathcal{S}_k \cup \mathcal{R}
\end{equation}



\begin{algorithm}[!t]
	\begin{algorithmic}
		\Require $\mathcal{M}_{k-1}, \mathcal{D}_{k}, \Phi_k$
		\\
        // Let $\omega_M^{(k-1)}$ be the procedure to select a subset of images from $\mathcal{M}_{k-1}$
        \\
        // Let $\omega_D^{(k)}$ be the procedure to select a subset of images from $\mathcal{D}_{k}$.
        \\
        \begin{comment}
        // Let $\mathcal{Q}$ be the transformer in the network
        \\
        // Let $\mathcal{W}$ be the MLP layers after the transformer in the network
        \\
        \end{comment}
		$\mathcal{M}_k \gets \omega_M^{(k-1)} \Bigl(\mathcal{M}_{k-1}\Bigr) \: \bigcup 
        \: \omega_D^{(k)}\Bigl(\mathcal{D}_{k}\Bigr)$
        \Repeat
            \State $\mathcal{L}_\psi \gets 0$
    		\For {$i = 1; \;\; i \leq |\mathcal{M}_k|; \;\; i \pluseq 1$}
                \State$I_i = \mathcal{M}_k\left[i\right]$
                \State $\mathbf{X} \gets \{\empty\}$
                \For {$\ell = 1; \;\; \ell \leq |\Phi_k|; \;\; \ell \pluseq 1$}
                    \State $\phi_{\ell} \gets \Phi_k\left[\ell\right]$
                    \State $\mathbf{X} \gets \mathbf{X} \cup \{\phi_{\ell}(I_i)\}$
                \EndFor
                \begin{comment}
    			\State $\mathbf{Z} \gets \mathcal{Q}(\mathbf{X})$
                \For {$j = 1; \;\; j \leq |\mathbf{Z}|; \;\; j \pluseq 1$}
                    \State $\ubar{z}{j} \gets \mathbf{Z}\left[j\right], \; \ubar{x}{j} \gets \mathbf{X}\left[j\right]$
                    \State $\ubar{z}{j} \gets \ubar{x}{j} \odot \ubar{z}{j}$ \Comment{$\odot$ is the Hadamard product}
                \EndFor
                \end{comment}
                \State $\hat{y}_i \gets \psi_k(\mathbf{X})$ % \Comment{$\hat{y}_i$ is detection score}
                \State $\mathcal{L}_\psi \gets \mathcal{L}_\psi - ( \hat{y}_i \log{(t_i)} + (1 - \hat{y}_i) \log{(1 - t_i)}) $
            \EndFor
            \State $\psi_k \gets \text{Back-propagate}(\mathcal{L}_\psi, \psi_k)$ 
        \Until {max epoch is reached}
        \\
        \Return $\psi_k$
	\end{algorithmic}
    \caption{\:\: Training \Reasoner} \label{alg:train_ekfn}
\end{algorithm}




\subheader{Training EKFN}
After constructing $\mathcal{M}_k$, we utilize it to train EKFN. Here, we refer to EKFN with the symbol $\psi$ to have a uniform notation. $\psi(\cdot)$ maps $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$ to a single binary detection decision. To do that, $\psi$ jointly processes the embeddings in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$ to utilize the most important information for making a detection decision for each input image.
To train this network, using the following loss function:
\begin{dmath}
    \label{eq:l_ekfn}
    \mathcal{L}_\psi = 
    \sum_{I_\ell \in \mathcal{M}_k} \psi(\{\ubar{x}{1}^\ell, \ldots, \ubar{x}{k}^\ell \}) \log{t_\ell} +
    (1 - \psi(\{\ubar{x}{1}^\ell, \ldots, \ubar{x}{k}^\ell \})) \log(1-t_\ell)
\end{dmath}
where $t_\ell$ is the ground-truth label for $I_\ell$, we optimize the weights of the network. The training procedure of EKFN is provided in Alg.~\ref{alg:train_ekfn}.

%$\psi$ maps $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$ needs to make a decision based on the sequence of embeddings, , which is produced by the embedders in $\Phi_k$ for each input image.

%, which we define as $\mathcal{L}_k = \{\ubar{x}{l} \: | \: \varphi_l \in \{ \phi_1, \ldots, \phi_k  \} \}$.

%We use $\psi$ to produce a vector $\ubar{z}{\ell}$ for each corresponding element in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$.


% \State $\mathbf{X} \gets \{   \phi_{\ell}(i) \: | \: \phi_{\ell} \in \Phi_k \}$
% \State $\mathbf{Z} \gets \{  \ubar{x}{l} \odot \ubar{z}{l} | \ubar{x}{l} \in \mathbf{X}, \ubar{z}{l} \in \mathbf{Z} \}$


\subheader{EKFN architecture}
To analyze the set of embeddings, $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$ we use a transformer to treat each input embedding as a token in a sequence of forensic evidence. The transformer's output associated with each of the embeddings, which we refer to as $\ubar{z}{\ell}$, contains information about the relevance of $\ubar{x}{\ell}$  with respect to itself and other embeddings in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$. Effectively, the transformer helps the subsequent layers by highlighting relevant and de-emphasizing less relevant information in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$. 
We then scale $\ubar{x}{\ell}$ by $\ubar{z}{\ell}$ using the Hadamard product (element-wise product), which will be denoted as $\odot$. Subsequently, we provide the sequence of scaled embeddings to a classifier network composed of only a few linear layers to generate a single detection decision for the input.
The network's architecture is depicted in Fig.~\ref{fig:overall_sys_diagram}.









==> sec/EKFN_v4_Tai.tex <==



\subsection{Training Expert Knowledge Fusion Network}
\label{subsec:ekfn_training}

After adding the expert embedder $\phi_k$ to the set of existing \ee, we train the Expert Knowledge Fusion Network (EKFN) to perform classification. This network aims to fuse the embeddings resulted from the application of all embedders in $\Phi_k$ on each input image, and subsequently, produce a final detection decision based on the joint knowledge of all embedders.
In the following, we first discuss the update procedure of the memory buffer in the face of emergence of a new generator. Then, we explain the training procedure of EKFN, and finally, we discuss the architecture we select to use as EKFN.

%In the following, we first discuss the architecture of EKFN. Then, we talk about how the memory buffer is updated when a new generator shows up, and finally explain the training procedure of EKFN.

% We will refer to the EKFN as $\psi$ in the following to have a uniform notation. To train $\psi$, we first need to update the memory buffer using $\mathcal{D}_k$. 


\subheader{Updating Memory Buffer}
%\label{subheader:mem}
To update memory buffer $\mathcal{M}_{k-1}$ to obtain $\mathcal{M}_k$, we use the same set of real data, $\mathcal{R}$, used to train $\phi_k$. However, to have a balanced representation of all known generators, we need to include a subset of $\mathcal{D}_k$ in the memory buffer. We form $\mathcal{S}_k$, the synthetic portion of $\mathcal{M}_k$, by retaining $P_k$ number of images from each generator, where $P_k$ is defined as follows:
\begin{equation}
    \small
    P_k = \floor*{\dfrac{M}{2(k+1)}}
\end{equation}
where $\floor{\cdot}$ denotes the floor function.

Therefore, after adding generator $g_k$, the number of synthetic images in $\mathcal{S}_k$ will be equal to $(k+1)P_k$, which is equal or close to ${M}/{2}$, as desired. Then, we construct $\mathcal{S}_k$ by pulling $P_k$ images per generator from $\mathcal{S}_{k-1}$ and $P_k$ images from $\mathcal{D}_k$. Effectively, $S_{k}$ consists of ${M}/{2}$ data points equally created by generators in $\mathcal{G}_k$. Finally, we define:

\begin{equation}
    \mathcal{M}_k = \mathcal{S}_k \cup \mathcal{R}
\end{equation}



\begin{algorithm}[!t]
	\begin{algorithmic}
		\Require $\mathcal{M}_{k-1}, \mathcal{D}_{k}, \Phi_k$
		\\
        // Let $\omega_M^{(k-1)}$ be the procedure to select a subset of images from $\mathcal{M}_{k-1}$
        \\
        // Let $\omega_D^{(k)}$ be the procedure to select a subset of images from $\mathcal{D}_{k}$.
        \\
        \begin{comment}
        // Let $\mathcal{Q}$ be the transformer in the network
        \\
        // Let $\mathcal{W}$ be the MLP layers after the transformer in the network
        \\
        \end{comment}
		$\mathcal{M}_k \gets \omega_M^{(k-1)} \Bigl(\mathcal{M}_{k-1}\Bigr) \: \bigcup 
        \: \omega_D^{(k)}\Bigl(\mathcal{D}_{k}\Bigr)$
        \Repeat
            \State $\mathcal{L}_\psi \gets 0$
    		\For {$i = 1; \;\; i \leq |\mathcal{M}_k|; \;\; i \pluseq 1$}
                \State$I_i = \mathcal{M}_k\left[i\right]$; \;$\mathbf{X} \gets \{\empty\}$
                \For {$j = 1; \;\; j \leq |\Phi_k|; \;\; j \pluseq 1$}
                    \State $\phi_{j} \gets \Phi_k\left[j\right]$
                    \State $\mathbf{X} \gets \mathbf{X} \cup \{\phi_{j}(I_i)\}$
                \EndFor
                \begin{comment}
    			\State $\mathbf{Z} \gets \mathcal{Q}(\mathbf{X})$
                \For {$j = 1; \;\; j \leq |\mathbf{Z}|; \;\; j \pluseq 1$}
                    \State $\ubar{z}{j} \gets \mathbf{Z}\left[j\right], \; \ubar{x}{j} \gets \mathbf{X}\left[j\right]$
                    \State $\ubar{z}{j} \gets \ubar{x}{j} \odot \ubar{z}{j}$ \Comment{$\odot$ is the Hadamard product}
                \EndFor
                \end{comment}
                \State $\hat{y}_i \gets \psi_k(\mathbf{X})$ % \Comment{$\hat{y}_i$ is detection score}
                \State $\mathcal{L}_\psi \gets \mathcal{L}_\psi - ( y_i \log{(\hat{y}_i)} + (1 - y_i) \log{(1 - \hat{y}_i)}) $
            \EndFor
            \State $\psi_k \gets \text{Back-propagate}(\mathcal{L}_\psi, \psi_k)$ 
        \Until {max epoch is reached}
        \\
        \Return $\psi_k$
	\end{algorithmic}
    \caption{\:\: Training \Reasoner} \label{alg:train_ekfn}
\end{algorithm}




\subheader{Training EKFN}
After constructing $\mathcal{M}_k$, we utilize it to train EKFN. Here, we refer to EKFN with the symbol $\psi$ to have a uniform notation. $\psi(\cdot)$ maps $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$ to a single binary detection decision. To do that, $\psi$ jointly processes the embeddings in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$ to utilize the most important information for making a detection decision for each input image.
To train this network, using the following loss function:
\begin{dmath}
    \label{eq:l_ekfn}
    \mathcal{L}_\psi = 
    \sum_{I_\ell \in \mathcal{M}_k} \psi(\{\ubar{x}{1}^\ell, \ldots, \ubar{x}{k}^\ell \}) \log{t_\ell} +
    (1 - \psi(\{\ubar{x}{1}^\ell, \ldots, \ubar{x}{k}^\ell \})) \log(1-t_\ell)
\end{dmath}
where $t_\ell$ is the ground-truth label for $I_\ell$, we optimize the weights of the network. The training procedure of EKFN is provided in Alg.~\ref{alg:train_ekfn}.



\subheader{EKFN architecture}
To analyze the set of embeddings, $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$ we use a transformer to treat each input embedding as a token in a sequence of forensic evidence. The transformer's output associated with each of the embeddings, which we refer to as $\ubar{z}{\ell}$, contains information about the relevance of $\ubar{x}{\ell}$  with respect to itself and other embeddings in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$. Effectively, the transformer helps the subsequent layers by highlighting relevant and de-emphasizing less relevant information in $\{\ubar{x}{1}, \ldots, \ubar{x}{k} \}$. 
We then scale $\ubar{x}{\ell}$ by $\ubar{z}{\ell}$ using the Hadamard product (element-wise product), which will be denoted as $\odot$. Subsequently, we provide the sequence of scaled embeddings to a classifier network composed of only a few linear layers to generate a single detection decision for the input.
The network's architecture is depicted in Fig.~\ref{fig:overall_sys_diagram}.









==> sec/ExpertEmbedder_v0.tex <==



\subsection{Training New Expert Embedder}
When a new synthetic image generator $g_{k > 0}$ emerges we need to make a new expert to capture traces associated with it. To do this, we utilize $\mathcal{D}_k$ and $\mathcal{R}$ to train an expert embeddor $\varphi_k$ through transfer learning.
%
Specifically, we fine-tune $f_0$ using $\mathcal{D}_k \cup \mathcal{R}$ to get an intermediate expert detector $\hat{f}_k$. This new detector will likely experience catastrophic forgetting and lose significant ability to detect generators other than $g_k$. Then, we extract expert embedder $\varphi_k$ by discarding the classification component $h_k$ of $\hat{f}_k$. This procedure is outlined in Alg.~\ref{alg:ft}. 

%After obtaining the expert embedder $\varphi_k$, we update $\mathcal{M}_{k-1}$ to $\mathcal{M}_{k}$, which will be used as the only training data for the classification sub-network. Additionally, we form $\mathcal{G}_k = \mathcal{G}_{k-1} \cup \{g_k\}$. (\red{we need to put these last two steps in the main algorithm probably}).

\begin{algorithm}
	\caption{\:\: Train $\varphi_k$}\label{alg:ft}
	\begin{algorithmic}[1]
		\Procedure{TrainExpert}{$f_0, \mathcal{D}_k, \mathcal{R}, \mathcal{P}$}
		\State Form $\mathcal{T} = \mathcal{D}_k \cup \mathcal{R}$
		\State Fine-tune $f_0$ with $\mathcal{T}$ to get $\hat{f}_k$ using $\mathcal{P}$
		\State Extract $\varphi_k$ by discarding $h_k$ of $\hat{f}_0$
		\State \Return $\varphi_k$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

==> sec/ExpertEmbedder_v1_MCS.tex <==
% ExpertEmbedder_v1_MCS
%
\subsection{Training New Expert Embedder}

When a new synthetic image generator emerges, we need to create a new expert embedder to capture its traces.  To accomplish this, we utilize transfer learning to adapt the baseline detector $f_0$ to create the new expert $\phi_k$.

The existing memory buffer $\mathcal{M}_{k-1}$ is composed of two subsets: an unchanging set of $M/2$ real images $\mathcal{R}$ as well as a set of $M/2$ synthetic images $\mathcal{S}_{k-1}$.

When a new synthetic image generator $g_{k > 0}$ emerges we need to make a new expert to capture traces associated with it. To do this, we utilize $\mathcal{D}_k$ and $\mathcal{R}$ to train an expert embeddor $\varphi_k$ through transfer learning.
%
Specifically, we fine-tune $f_0$ using $\mathcal{D}_k \cup \mathcal{R}$ to get an intermediate expert detector $\hat{f}_k$. This new detector will likely experience catastrophic forgetting and lose significant ability to detect generators other than $g_k$. Then, we extract expert embedder $\varphi_k$ by discarding the classification component $h_k$ of $\hat{f}_k$. This procedure is outlined in Alg.~\ref{alg:ft}. 

%After obtaining the expert embedder $\varphi_k$, we update $\mathcal{M}_{k-1}$ to $\mathcal{M}_{k}$, which will be used as the only training data for the classification sub-network. Additionally, we form $\mathcal{G}_k = \mathcal{G}_{k-1} \cup \{g_k\}$. (\red{we need to put these last two steps in the main algorithm probably}).

\begin{algorithm}
	\caption{\:\: Train $\varphi_k$}\label{alg:ft}
	\begin{algorithmic}[1]
		\Procedure{TrainExpert}{$f_0, \mathcal{D}_k, \mathcal{R}, \mathcal{P}$}
		\State Form $\mathcal{T} = \mathcal{D}_k \cup \mathcal{R}$
		\State Fine-tune $f_0$ with $\mathcal{T}$ to get $\hat{f}_k$ using $\mathcal{P}$
		\State Extract $\varphi_k$ by discarding $h_k$ of $\hat{f}_0$
		\State \Return $\varphi_k$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

==> sec/ExpertEmbedder_v2_Aref.tex <==
% ExpertEmbedder_v1_MCS
%
\subsection{Training New Expert Embedder}

If a new synthetic image generator emerges, we need to create a new expert embedder to capture its traces.  To accomplish this, we utilize transfer learning to adapt the baseline detector $f_0$ to create the new expert $\phi_k$.

%The existing memory buffer $\mathcal{M}$ is composed of two subsets: an unchanging set of $M/2$ real images $\mathcal{R}$ as well as a set of $M/2$ synthetic images $\mathcal{S}$.

At the emergence of a new synthetic image generator, $g_{k > 0}$, we utilize $\mathcal{D}_k$ and $\mathcal{R}$ to train an expert embedder $\phi_k$ through transfer learning. 
Specifically, we fine-tune $f_0$ using $\mathcal{D}_k \cup \mathcal{R}$ to get an intermediate expert detector $\hat{f}_k$. This new detector will likely experience catastrophic forgetting and lose significant ability to detect generators other than $g_k$. Then, we extract expert embedder $\phi_k$ by discarding the classification component $h_k$ of $\hat{f}_k$. This procedure is outlined in Alg.~\ref{alg:ft}.

%When a new synthetic image generator $g_{k > 0}$ emerges we need a new expert to capture the traces associated with it. To do this, we utilize $\mathcal{D}_k$ and $\mathcal{R}$ to train an expert embedder $\phi_k$ through transfer learning.
%
 

%After obtaining the expert embedder $\varphi_k$, we update $\mathcal{M}_{k-1}$ to $\mathcal{M}_{k}$, which will be used as the only training data for the classification sub-network. Additionally, we form $\mathcal{G}_k = \mathcal{G}_{k-1} \cup \{g_k\}$. (\red{we need to put these last two steps in the main algorithm probably}).

\begin{algorithm}
	\begin{algorithmic}[1]
		\Procedure{TrainExpert}{$f_0, \mathcal{D}_k, \mathcal{R}, \mathcal{P}$}
		\State Form $\mathcal{T} = \mathcal{D}_k \cup \mathcal{R}$
		\State Fine-tune $f_0$ with $\mathcal{T}$ to get $\hat{f}_k$ using $\mathcal{P}$
		\State Extract $\phi_k$ by discarding $h_k$ of $\hat{f}_k$
		\State \Return $\phi_k$
		\EndProcedure
	\end{algorithmic}
    \caption{\: \: Train $\phi_k$, $\mathcal{P}$ represents the training hyper-parameters} \label{alg:ft}
\end{algorithm}

==> sec/ExpertEmbedder_v3_MCS.tex <==
% ExpertEmbedder_v1_MCS
%
\subsection{Training New Expert Embedder}
\label{subsec:new_expert_training}

%When a new synthetic image generator emerges, we need to create a new expert embedder to capture its traces.  

%Let us assume that the current set of known synthetic image generators 

Let $\mathcal{G}_{k-1}$ be the set of currently known synthetic image generators.
%
When a new synthetic image generator $g_k\notin\mathcal{G}_{k-1}$ emerges, we need to update our detector. 
%We start by creating 
To do this, we must first create 
a new expert embedder $\phi_k$ to capture traces left by $g_k$.  We accomplish this by adapting the baseline detector $f_0$ using transfer learning.  

We start by forming a new expert training set $\mathcal{T}_k$ of real and synthetic images that we will use to create $\phi_k$. 
This is done by collecting a set $\mathcal{D}_k$ of $N$ synthetic images created by the new generator.
%
Real images are taken from the current memory buffer $\mathcal{M}_{k-1}$, which is composed of a set $\mathcal{R}$ of $M/2$ real images as well as a set $\mathcal{S}_{k-1}$ synthetic images made by generators in $\mathcal{G}_{k-1}$. 
(\red{don't we need to define $\mathcal{S}_0$ and $\mathcal{M}_0$?})
As a result, the new expert training set is
\begin{equation}
    \mathcal{T}_k= \mathcal{D}_k \cup \mathcal{R}.
\end{equation}

Next, we use $\mathcal{T}_k$ to update $f_0$ to detect images made by $g_k$.  Specifically, we form a new detector $\hat{f}_k$ by fine tuning $f_0$  with $\mathcal{T}_k$ using the loss function \textbf{DOUBLE CHECK AND CORRECT THIS}
\begin{dmath}
\mathcal{L}_\phi= \sum_{I\in \mathcal{T}_k} \tfrac{|\mathcal{D}_k|}{|\mathcal{T}_k|} t(I) log(\hat{f}_k(I)) + 
\tfrac{|\mathcal{R}|}{|\mathcal{T}_k|} (1-t(I)) log(1-\hat{f}_k(I))
\end{dmath}
where $|\cdot|$ denotes the set cardinality operator and $t$ is a class label such that $t(I)$ is 1 if the image is synthetic and 0 if it is real.

%NOTE BELOW CAN POTENTIALLY BE REMOVED
By doing this, the resulting detector $\hat{f}_k$ will be adapted to detect images made by $g_k$.  However, it will likely experience catastrophic forgetting and be poorly suited to detect generators in $\mathcal{G}_{k-1}$. \textbf{This paragraph can be removed if desired}

After obtaining the expert detector $\hat{f}_k$, we decompose it into its corresponding expert embedder $\phi_k$ and classifier components.  The classifier portion is discarded, while $\phi_k$ is retained. 
%
Finally, $\phi_k$ is added to the set of expert embedders $\Phi_k= \Phi_{k-1} \cup \{\phi_k\}$.  We note $\Phi_0$ is initialzed as $\Phi_0= \{\phi_0\}$.
%
This procedure is summarized in Alg.~\ref{alg:train_expert_emb}.

%When a new synthetic image generator $g_{k > 0}$ emerges we need a new expert to capture the traces associated with it. To do this, we utilize $\mathcal{D}_k$ and $\mathcal{R}$ to train an expert embedder $\phi_k$ through transfer learning.
%
 

%After obtaining the expert embedder $\varphi_k$, we update $\mathcal{M}_{k-1}$ to $\mathcal{M}_{k}$, which will be used as the only training data for the classification sub-network. Additionally, we form $\mathcal{G}_k = \mathcal{G}_{k-1} \cup \{g_k\}$. (\red{we need to put these last two steps in the main algorithm probably}).

\begin{algorithm}
	\begin{algorithmic}
        \Require $f_0, \mathcal{D}_k, \mathcal{R}$ 
        \\
		$\mathcal{T}_k \gets \mathcal{D}_k \cup \mathcal{R}$
        \\
        // Let $\Gamma_\ell$ be the fine-tuning procedure for the detector $f_\ell$ on the dataset $\mathcal{T}_k$: 
        \\
		$\hat{f}_k \gets \Gamma_\ell(f_0, \mathcal{T}_k)$
        \\
        // Since: $\hat{f}_k = h_k \circ \phi_k$
        \\
		\Return $\phi_k$
	\end{algorithmic}
    \caption{\: \: Training \Ee} \label{alg:train_expert_emb}
\end{algorithm}

==> sec/ExpertEmbedder_v4_Tai.tex <==
% ExpertEmbedder_v1_MCS
%
\subsection{Training New Expert Embedder}
\label{subsec:new_expert_training}
\input{figures/new_expert_training_v1_manil}
%When a new synthetic image generator emerges, we need to create a new expert embedder to capture its traces.  

%Let us assume that the current set of known synthetic image generators 

Let $\mathcal{G}_{k-1}$ be the set of currently known synthetic image generators.
%
When a new synthetic image generator $g_k\notin\mathcal{G}_{k-1}$ emerges, we need to update our detector. 
%We start by creating 
To do this, we must first create 
a new expert embedder $\phi_k$ to capture traces left by $g_k$.  We accomplish this by adapting the baseline detector $f_0$ using transfer learning.

Additionally, we note that the current memory buffer, $\mathcal{M}_{k-1}$, composes of two subsets, the set of real images $\mathcal{R}$, and the set of synthetic images $\mathcal{S}_{k-1}$ made by generators in $\mathcal{G}_{k-1}$. To simplify our setup, we assume that $|\mathcal{R}| = |\mathcal{S}_{k-1}| = M/2$.

Now we start by forming a new expert training set, $\mathcal{T}_k$, composes of real and synthetic images that we will use to create $\phi_k$. 
This is done by first collecting a set of $N$ synthetic images, $\mathcal{D}_k$, from the new generator, where $N \leq M/2$.
%
To complement this set of synthetic images, we take the set of real images $\mathcal{R}$ from the current memory buffer $\mathcal{M}_{k-1}$.
% (\red{don't we need to define $\mathcal{S}_0$ and $\mathcal{M}_0$?})
As a result, the new expert training set is defined as
\begin{equation}
    \mathcal{T}_k= \mathcal{D}_k \cup \mathcal{R}.
\end{equation}

Next, we use $\mathcal{T}_k$ to update $f_0$ to detect images made by $g_k$.  Specifically, we form a new detector $\hat{f}_k$ by fine tuning $f_0$  with $\mathcal{T}_k$ using the loss function 
% \textbf{DOUBLE CHECK AND CORRECT THIS}
\begin{align*}
    \mathcal{L}_\phi = - \sum_{I_\ell\in \mathcal{T}_k} 
    \frac{|\mathcal{D}_k|}{|\mathcal{T}_k|} y_\ell log(\hat{f}_k(I_\ell)) \\ + 
    \frac{|\mathcal{R}|}{|\mathcal{T}_k|} (1 - y_\ell) log(1-\hat{f}_k(I_\ell))
\end{align*}
where $|\cdot|$ denotes the set cardinality operator, $I_\ell$ is the $\ell$-th image in $\mathcal{T}_k$, and $y_\ell$ is the class label of the image $I_\ell$ where 0 means the image is real and 1 means the image is synthetic.

%NOTE BELOW CAN POTENTIALLY BE REMOVED
By doing this, the resulting detector $\hat{f}_k$ will be adapted to detect images made by $g_k$.  However, it will likely experience catastrophic forgetting and be poorly suited to detect generators in $\mathcal{G}_{k-1}$. 
% \textbf{This paragraph can be removed if desired}

After obtaining the expert detector $\hat{f}_k$, we decompose it into its corresponding expert embedder $\phi_k$ and classifier components. The classifier portion is discarded, while $\phi_k$ is retained. 
%
Finally, $\phi_k$ is added to the set of expert embedders $\Phi_k= \Phi_{k-1} \cup \{\phi_k\}$.  We note $\Phi_0$ is initialized as $\Phi_0= \{\phi_0\}$.
%
This procedure is summarized in Alg.~\ref{alg:train_expert_emb}.

%When a new synthetic image generator $g_{k > 0}$ emerges we need a new expert to capture the traces associated with it. To do this, we utilize $\mathcal{D}_k$ and $\mathcal{R}$ to train an expert embedder $\phi_k$ through transfer learning.
%
 

%After obtaining the expert embedder $\varphi_k$, we update $\mathcal{M}_{k-1}$ to $\mathcal{M}_{k}$, which will be used as the only training data for the classification sub-network. Additionally, we form $\mathcal{G}_k = \mathcal{G}_{k-1} \cup \{g_k\}$. (\red{we need to put these last two steps in the main algorithm probably}).

\begin{algorithm}
	\begin{algorithmic}
        \Require $f_0, \mathcal{D}_k, \mathcal{R}$ 
        \\
        // Form training dataset $\mathcal{T}_k$:
        \\
		$\mathcal{T}_k \gets \mathcal{D}_k \cup \mathcal{R}$
        \\
        // Let $\tau$ be the procedure for training $f_0$ on the dataset $\mathcal{T}_k$: 
        \\
		$\hat{f}_k \gets \tau(f_0, \mathcal{T}_k, \mathcal{L}_\phi)$
        \\
        Discard $h_k$, Keep $\phi_k$ only \; // $\hat{f}_k = h_k \circ \phi_k$
        \\
        $\Phi_k = \Phi_{k-1} \cup \{\phi_k\}$
        \\
		\Return $\Phi_k$
	\end{algorithmic}
    \caption{\: \: Training \Ee} \label{alg:train_expert_emb}
\end{algorithm}

==> sec/ProbForm_v1_MCS.tex <==
% ProbForm_v1_MCS
%
\section{Problem Formulation}

%Here we describe the general problem addressed in this paper.

We begin by assuming that an initial synthetic image detector $f_0$ has been created to detect images in a set of known generators $\gensetbl$.  We will refer to this detector as the baseline detector.  We further assume that $f_0$ was trained using a large baseline training dataset $\mathcal{B}$ consisting of both real and synthetic images in $\gensetbl$.

After the baseline detector has been trained, new synthetic image generators $g_k \notin \gensetbl$ will continue to emerge.  As previous research has shown, $f_0$ will have a difficult time detecting these generators if the forensic traces or ``fingerprints'' left by these generators are substantially different than those in left by the generators in $\gensetbl$~\cite{placeholder}. 
%$g_k \notin \gensetbl$
Because of this, the existing synthetic image detector will need to be updated with the emergence of new generators.

This presents a set of new problems. Training a new detector from scratch can be resource intensive and requires that the baseline dataset  $\mathcal{B}$ be stored indefinitely.  Instead, it is preferable to retain only a small dataset $\mathcal{M}$, known as the memory buffer, to update the the detector.  Similarly, it may not be feasible to access a large set of synthetic images from the new generator $g_k$.  For instance, the new generator may not be accessible to the general public, but a small number of examples from the generator may be publicly available.  An example of this is OpenAI's recently announced Sora generator~\cite{placeholder}.
In this case, the amount of images from the new generator that are available to update the detector may be limited. 

As a result, 
updating a synthetic detector in the presence of a new generator can be viewed as a continual learning problem.  
%It is important to note that con
To formalize this problem, we adopt terminology from the 
%In this paper, 
We define the memory buffer $\mathcal{M}_k$ available to retrain the detector when a new generator $g_k$ emerges has a fixed size $|\mathcal{M}_k|=N_1$.  We note that $N_1$ remains constant, even as more generators emerge.  As a result, images from the previous memory buffer $\mathcal{M}_{k-1}$ must be removed so that images from the new generator $g_k$ can be added to form  $\mathcal{M}_k$.  
%
\textbf{\textit{Should we say something about how different CL algorithms update M in a different manner?}}  
%
Additionally, we define the $\mathcal{D}_k$ as the set of images from the new generator $g_k$ that can be used to update the detector.  We similarly assume that this number is fixed for all new generators such that $|\mathcal{D}_k|=N_2$.


%Because the baseline dataset is large $\mathcal{B}$


==> sec/ProbForm_v2_MCS.tex <==
% ProbForm_v1_MCS
%
\section{Problem Formulation}

%Here we describe the general problem addressed in this paper.

We begin by assuming that an initial synthetic image detector $f_0$ has been created to detect images in a set of known generators $\gensetbl$.  We will refer to this detector as the baseline detector.  We further assume that $f_0$ was trained using a large baseline training dataset $\mathcal{B}$ consisting of both real and synthetic images in $\gensetbl$.

After the baseline detector has been trained, new synthetic image generators $g_k \notin \gensetbl$ will continue to emerge.  As previous research has shown, $f_0$ will have a difficult time detecting these new generators if the forensic traces or ``fingerprints'' left by these generators are substantially different than those left by the generators in $\gensetbl$~\cite{corvi2023detection}. 
%in left by the generators in $\gensetbl$~\cite{placeholder}. 
%$g_k \notin \gensetbl$
Because of this, the synthetic image detector will need to be continually updated as new generators emerge. 
%with the emergence of new generators.

This presents a set of new problems. Training a new detector from scratch can be resource intensive and requires that the baseline dataset  $\mathcal{B}$ be stored indefinitely.  Instead, it is preferable to retain only a small dataset $\mathcal{M}$, known as the memory buffer, to update the detector.  
%
Care must be taken when updating the detector, however, because naively fine-tuning the detector can lead to catastrophic forgetting.  When this happens, the detector is able to identify images produced by the new generator but loses the ability to reliably detect images from previous generators.
%using data from
%This can be challenging due to an issue known as catastrophic forgetting.  If 

Additionally, challenges may arise when access to synthetic images generated by the new generator $g_k$ is limited.  For instance, a generator may not be available to the general public, but a small number of examples from the generator may be publicly obtainable.  
%
% An example of this is OpenAI's recently announced Sora generator~\cite{sora}.  A small number of sample outputs from Sora have been shared with the public, however, access to Sora is currently restricted.  
An example of this is OpenAI's Sora generator~\cite{sora}, whose access is restricted but the company shared a small number of sample outputs. 
Alternatively, a party engaged in a misinformation campaign may have developed a new generator for their purposes. 
In this case, access to images produced by this new generator is severely limited by the
% it may be possible to identify a 
number of examples from which have been released into the wild.
% While this generator may not be accessible to produce training data, it may be possible to identify a number of examples from it which have been released into the wild using alternative investigations or open set detection and clustering approaches.
%
%In this case, , the amount of images from the new generator that are available to update the detector may be limited. 
% In these cases, the amount of data from the new generator that can be used to update the detector may be significantly limited.
As a result, developing an effective synthetic image detector, that can continuously adapt to new generators while having limited training data, is highly non-trivial.

%As a result, 
%Updating a synthetic detector in the presence of a new generator can be viewed as a continual learning problem.  
%It is important to note that con
%To formalize this problem, %we adopt terminology from the 
%In this paper, 

To formalize the problem of updating the detector given these constraints, we define the memory buffer $\mathcal{M}$ as the dataset of real images, and synthetic images from previously seen generators that is retained to update the detector.  The memory buffer has a fixed size $|\mathcal{M}|=M$ that remains constant, even as more generators emerge.  As a result, if images from a new generator are added to the memory buffer, a corresponding number of images must be removed.

Additionally, we define the $\mathcal{D}_k$ as the set of images from the new generator $g_k$ that can be used to update the detector.  We assume that this number is fixed for all new generators such that $|\mathcal{D}_k|=N$.  We further assume that $N$ is significantly smaller than the number of images in $\mathcal{B}$, i.e. we have only a limited number of images from a new generator that we can use to update the detector.

%we define the memory buffer $\mathcal{M}_k$ available to retrain the detector when a new generator $g_k$ emerges has a fixed size $|\mathcal{M}_k|=N_1$.  We note that $N_1$ remains constant, even as more generators emerge.  As a result, images from the previous memory buffer $\mathcal{M}_{k-1}$ must be removed so that images from the new generator $g_k$ can be added to form  $\mathcal{M}_k$.  
%
%\textbf{\textit{Should we say something about how different CL algorithms update M in a different manner?}}  
%
%Additionally, we define the $\mathcal{D}_k$ as the set of images from the new generator $g_k$ that can be used to update the detector.  We similarly assume that this number is fixed for all new generators such that $|\mathcal{D}_k|=N_2$.


%Because the baseline dataset is large $\mathcal{B}$


==> sec/ProbForm_v3_Tai.tex <==
% ProbForm_v1_MCS
%
\section{Problem Formulation}

%Here we describe the general problem addressed in this paper.

We begin by assuming that an initial synthetic image detector $f_0$ has been created to detect images in a set of known generators $\gensetbl$.  We will refer to this detector as the baseline detector.  We further assume that $f_0$ was trained using a large baseline training dataset $\mathcal{B}$ consisting of both real and synthetic images in $\gensetbl$.

After the baseline detector has been trained, new synthetic image generators $g_k \notin \gensetbl$ will continue to emerge.  As previous research has shown, $f_0$ will have a difficult time detecting these new generators if the forensic traces or ``fingerprints'' left by these generators are substantially different than those left by the generators in $\gensetbl$~\cite{corvi2023detection}. 
%in left by the generators in $\gensetbl$~\cite{placeholder}. 
%$g_k \notin \gensetbl$
Because of this, the synthetic image detector will need to be continually updated as new generators emerge. 
%with the emergence of new generators.

This presents a set of new problems. Training a new detector from scratch can be resource intensive and requires that the baseline dataset  $\mathcal{B}$ be stored indefinitely.  Instead, it is preferable to retain only a small dataset $\mathcal{M}$, known as the memory buffer, to update the detector.  
%
Care must be taken when updating the detector, however, because naively fine-tuning the detector can lead to catastrophic forgetting.  When this happens, the detector is able to identify images produced by the new generator but loses the ability to reliably detect images from previous generators.
%using data from
%This can be challenging due to an issue known as catastrophic forgetting.  If 

Additionally, challenges may arise when access to synthetic images generated by the new generator $g_k$ is limited.  For instance, a generator may not be available to the general public, but a small number of examples from the generator may be publicly obtainable.  
%
% An example of this is OpenAI's recently announced Sora generator~\cite{sora}.  A small number of sample outputs from Sora have been shared with the public, however, access to Sora is currently restricted.  
An example of this is OpenAI's Sora generator~\cite{sora}, whose access is restricted but the company shared a small number of sample outputs. 
Alternatively, a party engaged in a misinformation campaign may have developed a new generator for their purposes. 
In this case, access to images produced by this new generator is severely limited by the
% it may be possible to identify a 
number of examples from which have been released into the wild.
% While this generator may not be accessible to produce training data, it may be possible to identify a number of examples from it which have been released into the wild using alternative investigations or open set detection and clustering approaches.
%
%In this case, , the amount of images from the new generator that are available to update the detector may be limited. 
% In these cases, the amount of data from the new generator that can be used to update the detector may be significantly limited.
As a result, developing an effective synthetic image detector, that can continuously adapt to new generators while having limited training data, is highly non-trivial.

%As a result, 
%Updating a synthetic detector in the presence of a new generator can be viewed as a continual learning problem.  
%It is important to note that con
%To formalize this problem, %we adopt terminology from the 
%In this paper, 

To formalize the problem of updating the detector given these constraints, we define the memory buffer $\mathcal{M}$ (\red{we already defined it above, is this necessary?}) as the dataset of real images, and synthetic images from previously seen generators that is retained to update the detector.  The memory buffer has a fixed size $|\mathcal{M}| \: = M$, where $|\cdot|$ is the cardinality operator, that remains constant, even as more generators emerge.  
%As a result, if images from a new generator are added to the memory buffer, a corresponding number of images must be removed.

Additionally, we define the $\mathcal{D}_k$ as the set of images from the new generator $g_k$ that can be used to update the detector.  We assume that this number is fixed for all new generators such that $|\mathcal{D}_k|=N$.  
% We further assume that $N$ is significantly smaller than the number of images in $\mathcal{B}$, 
We further assume that $N \ll |\mathcal{B}|$.
% i.e. the number of images from a new generator that we can use to update the detector is .

%we define the memory buffer $\mathcal{M}_k$ available to retrain the detector when a new generator $g_k$ emerges has a fixed size $|\mathcal{M}_k|=N_1$.  We note that $N_1$ remains constant, even as more generators emerge.  As a result, images from the previous memory buffer $\mathcal{M}_{k-1}$ must be removed so that images from the new generator $g_k$ can be added to form  $\mathcal{M}_k$.  
%
%\textbf{\textit{Should we say something about how different CL algorithms update M in a different manner?}}  
%
%Additionally, we define the $\mathcal{D}_k$ as the set of images from the new generator $g_k$ that can be used to update the detector.  We similarly assume that this number is fixed for all new generators such that $|\mathcal{D}_k|=N_2$.


%Because the baseline dataset is large $\mathcal{B}$


==> sec/ProbForm_v4_MCS.tex <==
% ProbForm_v4_MCS
%
\section{Problem Formulation}

%Here we describe the general problem addressed in this paper.

YeahWe begin by assuming that an initial synthetic image detector $f_0$ has been created to detect images in a set of known generators $\gensetbl$.  We will refer to this detector as the baseline detector.  We further assume that $f_0$ was trained using a large baseline training dataset $\mathcal{B}$ consisting of both real and synthetic images 
made using generators 
in $\gensetbl$.

After the baseline detector has been trained, new synthetic image generators $g_k \notin \gensetbl$ will continue to emerge.  As previous research has shown, $f_0$ will have a difficult time detecting these new generators if the forensic traces or ``fingerprints'' left by these generators are substantially different than those left by the generators in $\gensetbl$~\cite{corvi2023detection}. 
%in left by the generators in $\gensetbl$~\cite{placeholder}. 
%$g_k \notin \gensetbl$
Because of this, the synthetic image detector will need to be continually updated as new generators emerge. 
%with the emergence of new generators.

%This presents a set of %new 
This presents an important set of 
problems. Training a new detector from scratch can be resource intensive and requires that the baseline dataset  $\mathcal{B}$ be stored indefinitely.  Instead, it is preferable to retain only a small dataset $\mathcal{M}$, known as the memory buffer, to update the detector.  
%
Care must be taken when updating the detector, however, because naively fine-tuning the detector can lead to catastrophic forgetting.  When this happens, the detector is able to identify images produced by the new generator, but loses its ability to reliably detect images from previous generators.
%using data from
%This can be challenging due to an issue known as catastrophic forgetting.  If 

Additionally, challenges may arise when access to synthetic images generated by the new generator $g_k$ is limited.  For instance, a generator may not be available to the general public, but a small number of examples from the generator may be publicly obtainable.  
%
% An example of this is OpenAI's recently announced Sora generator~\cite{sora}.  A small number of sample outputs from Sora have been shared with the public, however, access to Sora is currently restricted.  
An example of this is OpenAI's Sora generator~\cite{sora}.
Currently, access to Sora is restricted, however OpenAI has shared a small number of sample outputs. 
%whose access is restricted but the company shared a small number of sample outputs. 
Alternatively, a party engaged in a misinformation campaign may have developed a new generator for their purposes. 
In this case, access to images produced by this new generator is severely limited by the
% it may be possible to identify a 
%
%number of examples from which have been released into the wild.
number of examples that have been released into the wild.
%can be  which have been released into the wild.
%
% While this generator may not be accessible to produce training data, it may be possible to identify a number of examples from it which have been released into the wild using alternative investigations or open set detection and clustering approaches.
%
%In this case, , the amount of images from the new generator that are available to update the detector may be limited. 
% In these cases, the amount of data from the new generator that can be used to update the detector may be significantly limited.
%As a result, developing an effective synthetic image detector, that can continuously adapt to new generators while having limited training data, is highly non-trivial.
Training an effective synthetic image detector that can continuously adapt to new generators with limited data 
%in cases such as these 
is highly non-trival.



%As a result, 
%Updating a synthetic detector in the presence of a new generator can be viewed as a continual learning problem.  
%It is important to note that con
%To formalize this problem, %we adopt terminology from the 
%In this paper, 

To formalize the problem of updating the detector given these constraints, we define $\prevbuf$ as the memory buffer when the $k^{th}$ new generator is introduced. $\prevbuf$ consists of two subsets: $\realset$ which contains real images and $\prevsynthset$ which contains images made by each of the previously seen generators.
The memory buffer has a fixed size $|\mathcal{M}_\ell|=M$ that remains constant even as more generators emerge.  
%As a result, if images from a new generator are added to the memory buffer, a corresponding number of images must be removed.
%
Additionally, we define the $\mathcal{D}_k$ as the set of images from the new generator $g_k$ that can be used to update the detector.  
%We assume that this number is fixed for all new generators such that $|\mathcal{D}_k|=N$.  
We assume that  $|\newdata|=N$ and that $N$ is significantly smaller than the number of images in $\mathcal{B}$, 
i.e. we have access to only have a limited number of images from the new generator to update the detector.
%
% We further assume that $N$ is significantly smaller than the number of images in $\mathcal{B}$, 
%We further assume that $N \ll |\mathcal{B}|$.
% i.e. the number of images from a new generator that we can use to update the detector is .

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hrulefill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
To formalize the problem of updating the detector given these constraints, we define the memory buffer $\mathcal{M}$ (\red{we already defined it above, is this necessary?}) as the dataset of real images, and synthetic images from previously seen generators that is retained to update the detector.  The memory buffer has a fixed size $|\mathcal{M}| \: = M$, where $|\cdot|$ is the cardinality operator, that remains constant, even as more generators emerge.  
%As a result, if images from a new generator are added to the memory buffer, a corresponding number of images must be removed.

Additionally, we define the $\mathcal{D}_k$ as the set of images from the new generator $g_k$ that can be used to update the detector.  We assume that this number is fixed for all new generators such that $|\mathcal{D}_k|=N$.  
% We further assume that $N$ is significantly smaller than the number of images in $\mathcal{B}$, 
We further assume that $N \ll |\mathcal{B}|$.
% i.e. the number of images from a new generator that we can use to update the detector is .

%we define the memory buffer $\mathcal{M}_k$ available to retrain the detector when a new generator $g_k$ emerges has a fixed size $|\mathcal{M}_k|=N_1$.  We note that $N_1$ remains constant, even as more generators emerge.  As a result, images from the previous memory buffer $\mathcal{M}_{k-1}$ must be removed so that images from the new generator $g_k$ can be added to form  $\mathcal{M}_k$.  
%
%\textbf{\textit{Should we say something about how different CL algorithms update M in a different manner?}}  
%
%Additionally, we define the $\mathcal{D}_k$ as the set of images from the new generator $g_k$ that can be used to update the detector.  We similarly assume that this number is fixed for all new generators such that $|\mathcal{D}_k|=N_2$.


\end{comment}

%Because the baseline dataset is large $\mathcal{B}$


==> sec/ProposedOverview_v1_MCS.tex <==



\section{Proposed Approach}
\label{sec:proposed_approach}
% ProposedOverview_v1_MCS

%Continual learning techniques typically address the problem of updating a network such 

While a synthetic image detector $f$ is often thought of as a single network, we can conceptually view it as the composition of an embedder $\phi$ and a classifier $h$, such that $f=h\circ\phi$. 
%In this view, the embedder produces an embedding that captures the forensic traces left synthetic image generators, while the detector maps these embeddings into detection decisions.
When adopting this view, the embeddings produced by $\phi$ capture forensic traces left by synthetic image generators, while the detector maps these embeddings to detection decisions. 
In practice, lower layers of the network can be thought of as the embedder, while the final layer or layers can be thought of as the classifier.  



% Continual learning techniques designed to update arbitrary networks used in AI and computer vision typically operate 

%Typically, continual learning techniques update 

%When continual learning techniques are used to update a synthetic image detector, this typically corresponds t \


When a continual learning technique is used to update %a synthetic image detector
$f$, this typically involves using a special process that retrains $f$ to  detect images from both a new generator and existing generators using $\mathcal{M}$ and $\mathcal{D}_k$.  
This corresponds to updating $\phi$ so that it learns an embedding space that is able to jointly capture forensic traces from previous generators as well as the new generator.  However, learning an embedding space that successfully does this can be challenging since the amount of data in $\mathcal{M}$ and $\mathcal{D}_k$ is limited.


To overcome this challenge, we propose a new approach to update $f$ which we call \textit{\Algname} (E3). In this approach, we do not attempt to learn a single embedding space to capture the traces left by all generators.  Instead, we create a set of expert embedders $\phi_k$ whose embedding space $\mathcal{X}_k$ is able to accurately capture traces from generator $g_k$.  We allow $\phi_k$ to experience catastrophic forgetting, since other experts in the ensemble are dedicated to capturing traces left by other generators.  
%As a result, we do not force the detector to learn a single embedding space that must be able to capture the traces left by all generators.  
%Instead, we create a set of embedding spaces ${\mathcal{X}_0,\ldots,\mathcal{X}_K}$ 
An image is analyzed by the entire ensemble of expert embedders to produce a sequence of embeddings $\{\ubar{x}{0},\ldots,\ubar{x}{k}\}$ that capture evidence that an image was created using generator $g_k$.  The sequence of embeddings is then analyzed using an Expert Knowledge Fusion Network (EKFN) to produce a single detection decision.  
%
As a result, traces from a generator do not need to be captured in a single embedding space, but in the union of the embedding spaces of all of our experts. 
%
%This network 
The expert knowledge fusion network takes the place of $h$ and can be trained using the limited data available in $\mathcal{M}$. 

We describe the process to form each expert embedder, update the memory buffer, and train the expert knowledge fusion network in the following subsections.

%By adopting this approach, we do not force the detector to learn a single embedding space that must be able to capture the traces left by all generators.  Instead, we create a set of embedding spaces ${\mathcal{X}_0,\ldots,\mathcal{X}_K$

==> sec/ProposedOverview_v2_Tai.tex <==



\section{Proposed Approach}
\label{sec:proposed_approach}
% ProposedOverview_v1_MCS

%Continual learning techniques typically address the problem of updating a network such 

While a synthetic image detector $f$ is often thought of as a single network, we can conceptually view it as the composition of an embedder $\phi$ and a classifier $h$, such that $f=h\circ\phi$. 
%In this view, the embedder produces an embedding that captures the forensic traces left synthetic image generators, while the detector maps these embeddings into detection decisions.
When adopting this view, the embeddings produced by $\phi$ capture forensic traces left by synthetic image generators, while the detector maps these embeddings to detection decisions. 
In practice, lower layers of the network can be thought of as the embedder, while the final layer or layers can be thought of as the classifier.  



% Continual learning techniques designed to update arbitrary networks used in AI and computer vision typically operate 

%Typically, continual learning techniques update 

%When continual learning techniques are used to update a synthetic image detector, this typically corresponds t \


When a continual learning technique is used to update %a synthetic image detector
$f$, this typically involves using a special process that retrains $f$ to  detect images from both a new generator and existing generators using $\mathcal{M}$ and $\mathcal{D}_k$.  
This corresponds to updating $\phi$ so that it learns an embedding space that is able to jointly capture forensic traces from previous generators as well as the new generator.  However, learning an embedding space that successfully does this can be challenging since the amount of data in $\mathcal{M}$ and $\mathcal{D}_k$ is limited.


To overcome this challenge, we propose a new approach to update $f$ which we call \textit{\Algname} (E3). In this approach, we do not attempt to learn a single embedding space to capture the traces left by all generators.  Instead, we create a set of expert embedders $\phi_k$ whose embedding space $\mathcal{X}_k$ is able to accurately capture traces from generator $g_k$.  We allow $\phi_k$ to experience catastrophic forgetting, since other experts in the ensemble are dedicated to capturing traces left by other generators.  
%As a result, we do not force the detector to learn a single embedding space that must be able to capture the traces left by all generators.  
%Instead, we create a set of embedding spaces ${\mathcal{X}_0,\ldots,\mathcal{X}_K}$

To analyze an input image, 
each expert embedder in the ensemble produces an embedding to form
a set of embeddings $\{\ubar{x}{0},\ldots,\ubar{x}{k}\}$ 
that capture evidence about the source of the input image.  
This set of embeddings is then analyzed using an Expert Knowledge Fusion Network (EKFN) to produce a single detection decision.  
%
As a result, our approach is able to leverage the union of the embedding spaces of all of our experts to capture traces from every generator.

We describe the process to form each expert embedder, update the memory buffer, and train the expert knowledge fusion network in the following subsections.

%By adopting this approach, we do not force the detector to learn a single embedding space that must be able to capture the traces left by all generators.  Instead, we create a set of embedding spaces ${\mathcal{X}_0,\ldots,\mathcal{X}_K$




% the traces from a generator do not need to be captured in a single embedding space, but in the union of the embedding spaces of all of our experts. 
%
%This network 

% The expert knowledge fusion network takes the place of $h$ and can be trained using the limited data available in $\mathcal{M}$. 










==> sec/ProposedSummary_v0.tex <==
\subsection{Summary}
To sum up, we perform the following steps in order to produce a synthetic image detector $f_k$ after the emergence of $g_k$, a new synthetic image generator. First, we fine-tune the baseline detector $f_0$ with a small amount of data generated by $g_k$ to create $\phi_k$, which we add to the set of existing expert embedders, $\mathcal{E}$. 
Additionally, we update $\mathcal{M}$ using $\mathcal{D}_k$, a small set of images generated by $g_k$. In order to maintain a balanced representation of each generator in $\mathcal{M}$, we use a uniformly random sampling strategy to sample an equal amount of data from each generator.
We then employ $\mathcal{E}$ to generate a sequence of embeddings for each data point in $\mathcal{M}$ and feed them to the transformer. Next, we scale the embeddings with the transformer's outputs using Hadamard product and use a few linear layers to output the final decision. Finally, we calculate a binary cross-entropy loss based on the network's decision and the ground-truth labels and use back-propagation to update EKFN's weights.

% \begin{algorithm}
% 	\caption{\:\: Train $f_k$}\label{alg:get_fk}
% 	\begin{algorithmic}[1]
% 		\Procedure{$\tau_3$}{$f_0, \mathcal{D}_k, \mathcal{R}, \mathcal{P}$}
% 		\EndProcedure
% 	\end{algorithmic}
% \end{algorithm}

==> sec/ablations_v0.tex <==
\input{tables/ablation_exp}

\section{Ablation Results}
\label{sec:ablations}
To understand the effects of components within the Expert Knowledge Fusion Network (EKFN), we conducted an ablation study; the results are presented in Table \ref{tab:ablation}.

\subheader{No Knowledge Fusion Net}
In this setting we removed the entire Knowledge Fusion NEtwork and employed a majority voting strategy, wherein each expert embedder retains its classification head during training. The output logits from these classifiers are summed and passed through a softmax activation to obtain predictions. This approach is akin to the proportional majority voting system detailed in previous research by \textcolor{red}{[FILL AND CITE]}. We can see that \textcolor{red}{[FILL THIS AFTER RESULTS ARE IN.]}

\subheader{Fusion with MLP only}
We also evaluated the EKFN without a transformer layer, meaning the embeddings themselves are fed directly into the final MLP layer. This variant confirmed that including a transformer layer positively impacts the model's performance.

\subheader{No Transformer Weighting}
The ``No Transformer Weighting'' refers to the exclusion of a residual connection to the transformer's output, leaving the MLP layer to process only the transformer's output. The findings suggest that incorporating embeddings with the transformer's output positively affects both accuracy and AUC.

\subheader{With Transformer Layers}
Our base architecture is the EKFN with a 5-layer transformer. The embeddings produced by $\phi_0, \ldots, \phi_k$ are provided as input to the transformer model. The output of the transformer is then combined with the residual data and fed into an MLP network for classification. Experiments indicate that optimal performance is achieved when a 5-layer transformer is incorporated into the EKFN. There is a noticeable, though slight, performance decline when the number of transformer layers is increased to 10.


==> sec/abstract_v0.tex <==
\begin{abstract}

Recent advances in generative artificial intelligence have sparked a revolution, leading to a surge of rapidly emerging techniques that produce high-quality and realistic images.
%
Traditional detection methods face two main challenges in adapting to these generators: 
%
the forensic traces of synthetic images from new techniques can vastly differ from those learned during training, 
%
and access to data for these new generators is often limited.
%
To address these issues, we introduce the Ensemble of Expert Embedders (E3), a novel continual learning framework for updating synthetic image detectors. E3 enables the accurate detection of images from newly emerged generators using minimal training data.
%
Our approach does this by first employing transfer learning to develop a suite of expert embedders, each specializing in the forensic traces of a specific generator. 
%
Then, all embeddings are jointly analyzed by an Expert Knowledge Fusion Network to produce accurate and reliable detection decision.
%
Our experiments demonstrate that E3 outperforms existing continual learning methods, including those developed specifically for synthetic image detection. 
Additionally, our results show that E3 is a general framework that can be applied across multiple detector architectures.

% E3 presents a novel and effective approach for continually updating synthetic image detectors in response to emerging generation techniques.



\end{abstract}


%%% Auto-Generated by ChatGPT %%%
%In the rapidly evolving landscape of synthetic image generation, traditional detectors struggle to keep pace with the emergence of new generators, leading to significant challenges in the field of image forensics. These challenges are exacerbated by the limitations of small training data size for new generators and the phenomenon of catastrophic forgetting, where updating a detector for new generators impairs its ability to recognize images from previously encountered generators. In this paper, we introduce a novel approach, \textit{\Algname} (E3), to address these challenges. Our method first reconceptualizes the synthetic image detector as a dynamic ensemble of expert embedders, each specialized in identifying the forensic traces of specific image generators. Unlike traditional approaches that seek to learn a universal embedding space for all generators, our method allows individual ``expert'' embedders to focus on distinct generators, thereby avoiding catastrophic forgetting and leveraging limited available data more effectively. By integrating these specialized embeddings through an expert knowledge fusion network, our system achieves robust and consistent detection across a wide spectrum of synthetic images, demonstrating superior adaptability and efficiency in handling the continual emergence of new synthetic image generators.

==> sec/abstract_v1_Tai.tex <==
\begin{abstract}

As generative AI progresses rapidly, new synthetic image generators continue to emerge at a swift pace. 
%
Traditional detection methods face two main challenges in adapting to these generators: 
%
the forensic traces of synthetic images from new techniques can vastly differ from those learned during training, 
%
and access to data for these new generators is often limited.
%
To address these issues, we introduce the Ensemble of Expert Embedders (E3), a novel  framework for updating synthetic image detectors. E3 enables the accurate detection of images from newly emerged generators using minimal training data.
%
Our approach does this by first employing transfer learning to develop a suite of expert embedders, each specializing in the forensic traces of a specific generator. 
%
Then, all embeddings are jointly analyzed by an Expert Knowledge Fusion Network to produce accurate and reliable detection decision.
%
Our experiments demonstrate that E3 outperforms existing continual learning methods, including those developed specifically for synthetic image detection. 
%
Additionally, our results show that E3 is a general framework that can be applied across multiple detector architectures.

% E3 presents a novel and effective approach for continually updating synthetic image detectors in response to emerging generation techniques.



\end{abstract}

==> sec/background_v0.tex <==
\section{Background}

\textbf{\red{Work in Progress}}

\label{sec:background}
 In 2006, Hinton et al. introduced Deep Belief Networks (DBNs), which probabilistically learned to reconstruct input data.\cite{hinton2006fast} This early work laid the groundwork for significant advancements in the field of generative models. In 2013, Kingma and Welling introduced the Variational Autoencoder (VAE), which quickly became popular for image generation.\cite{kingma2013auto} Subsequently, Generative Adversarial Networks (GANs) were proposed by Goodfellow et al., marking a seminal contribution to the field of synthetic image generation. \cite{goodfellow2014generative} Following the advent of GANs, numerous enhancements and variations have emerged, including Conditional GAN, CycleGAN, StyleGAN, Pix2Pix and BigGAN \cite{brock2018large,mirza2014conditional,zhu2017unpaired,isola2017image,karras2019style}. These models notably improved the quality, resolution, and realism of generated images, facilitating applications in art creation, photo-realistic image synthesis, and the generation of non-existent human faces.
 
 Diffusion models represent the current state-of-the-art in generating synthetic images. The concept of diffusion, widely recognized in physics, was first applied to image generation by Sohl-Dickstein et al., who introduced models that utilize stochastic processes. Specifically, these models employ a forward diffusion process to incrementally add noise to data and a reverse diffusion process to generate data from noise, drawing inspiration from thermodynamic principles.\cite{sohl2015deep} A subsequent 2020 paper by Ho et al. significantly advanced the field. \cite{ho2020denoising} Since these foundational contributions, diffusion models have undergone rapid development, with a variety of variants being proposed. Included among these are Latent Diffusion Models, along with innovations like Stable Diffusion, DALL·E, and Midjourney, which have continued to revolutionize image generation, yielding outputs that are both highly realistic and creatively rich based on textual descriptions or various inputs.\cite{rombach2022high,ramesh2021zero,zhang2023adding}
 

\subheader{Synthetic Image Detection}

Talk about a couple of papers (Detecting and simulating artifacts in gan fake images, cnn generated images are easy to spot, Deep Image Fingerprint:
Towards Low Budget Synthetic Image Detection and Model Lineage Analysis, etc.)

\subheader{Synthetic Image Forensic Traces}
Talk about how forensic traces left by different generators are distinct, you can cite this paper: On the detection of synthetic images generated by diffusion models, also I think it's useful to look at their background section

\subheader{Updating Synthetic Image Detectors}
Talk about other works directly related to us, like MTMC paper. I also found this one before: 
Cored: Generalizing fake media detection with continual representation using distillation
. Try to find another one but it's possible that there are no others.

\subheader{Continual Learning For Synthetic Image Detection}
Talk about continual learning, different general continual learning methods and that we can apply them to our problem and how?




==> sec/background_v1.tex <==
\section{Background}

\textbf{\red{Work in Progress}}

\label{sec:background}
 Since the introduction of Deep Belief Networks (DBNs) by Hinton \etal. in 2006~\cite{hinton2006fast}, generative models have undergone significant evolution, paving the way for groundbreaking developments in image generation. Variational Autoencoders (VAEs) in 2013 by Kingma and Welling~\cite{kingma2013auto}, and Generative Adversarial Networks (GANs) by Goodfellow \etal in 2014~\cite{goodfellow2014generative}, notably advanced the field, enhancing the quality and realism of synthetic images. Innovations such as Conditional GAN, CycleGAN, StyleGAN, Pix2Pix, and BigGAN further diversified applications and improved image fidelity~\cite{brock2018large,mirza2014conditional,zhu2017unpaired,isola2017image,karras2019style}.
 
 The breakthrough of diffusion models by Sohl-Dickstein \etal~\cite{sohl2015deep}, using stochastic processes for image creation, set new benchmarks in the generative landscape, significantly refined by Ho \etal in 2020~\cite{ ho2020denoising}. Presently, models like Latent Diffusion, Stable Diffusion, DALL·E, and Midjourney are generating highly detailed and imaginative visuals from various inputs, illustrating the generative models' expansive capabilities~\cite{rombach2022high,ramesh2021zero,zhang2023adding}. This progression reflects the field’s advancement towards creating synthetic imagery that closely mirrors real-life complexity, showcasing unprecedented artificial creativity and realism.
 

\subheader{Synthetic Image Detection}
%Talk about a couple of papers (Detecting and simulating artifacts in gan fake images, cnn generated images are easy to spot, Deep Image Fingerprint:
%Towards Low Budget Synthetic Image Detection and Model Lineage Analysis, etc.)
The detection of synthetic images plays a pivotal role in preserving the authenticity and reliability of digital media, which is essential for upholding individual privacy, ensuring security measures, and protecting intellectual property rights. With the rapid advancements in artificial intelligence technologies, there has been a significant increase in the capability to create highly realistic synthetic images, videos, and audio.  \\
Numerous efforts have been undertaken to distinguish synthetic images from real ones.  The works of Marra \etal~\cite{marra2019gans} have shown that GAN-generated images leave unique 'fingerprints', which can significantly enhance forensic analyses by facilitating source identification, distinguishing between real and synthetic content, and investigating the influence of network architecture and training datasets on these distinct identifiers. In 2019, Zhang \etal~\cite{zhang2019detecting} introduced AutoGAN, a GAN simulator that identifies up-sampling artifacts in the frequency domain, allowing for the training of a spectrum-based classifier on simulated images, which achieves superior detection of fake images without needing specific GAN-generated examples, which significantly improved classifier generalization. Subsequently, Wang \etal~\cite{wang2020cnn} discovered that image classifiers, rigorously fine-tuned with pre- and post-processing techniques and data augmentation, could generalize effectively to detect CNN based synthetic images across different generators, datasets, and methods, suggesting common flaws in CNN-generated images that limit realistic synthesis.
More recently, Sinitsa and Fried~\cite{sinitsa2024deep} developed a novel detection method, DIF, utilizing CNN architectural properties to extract image fingerprints, enabling the detection of synthetic images from specific models, including GANs and LTIMs based on Diffusion Models.

\subheader{Synthetic Image Forensic Traces}
%Talk about how forensic traces left by different generators are distinct, you can cite this paper: On the detection of synthetic images generated by diffusion models, also I think it's useful to look at their background section. Also, Learning and analyzing gan fingerprints.
[Need formal definition of forensic traces]Synthetic image forensic traces refers to the distinct, identifiable patterns, artifacts, or signatures left in images generated by synthetic image creation methods. It has been shown by numerous studies that every technique employed to generate synthetic visual content introduces specific traces into the resulting images, which are linked to the steps involved in the creation process~\cite{corvi2023detection, marra2019gans, yu2019attributing}. Prior works have also shown that different generator families leave significantly distinct forensic traces. The research by Corvi \etal demonstrates that unique generator types, such as GANs and diffusion models (DMs), produce specific forensic signatures. This emphasizes the challenge in developing detection methods capable of generalizing across types, especially highlighting the inadequacy of detectors trained exclusively on GAN images to accurately identify images generated by DMs~\cite{corvi2023detection}.


\subheader{Continual Learning For Synthetic Image Detection}
%Talk about continual learning, different general continual learning methods and that we can apply them to our problem and how?
Given the unique forensic traces produced by different generator families, it is essential for detectors to incrementally incorporate knowledge about new generators. Retraining the detector by storing images from both newer unseen generators and known ones is impractical due to the ever-increasing volume of images as new generators emerge. An alternative and more viable strategy is to finetune the existing detector with images generated by previously unknown models. However, this approach introduces the well-documented problem of catastrophic forgetting within the machine learning community. Catastrophic forgetting occurs in neural networks when they are exposed to data from a different distribution, resulting in a significant decline in performance on tasks they previously learned as the model shifts its focus to new tasks~\cite{mccloskey1989catastrophic, mcclelland1995there}. 

Considerable efforts have been dedicated to addressing these challenges by enabling models to learn continually, a process known as continual or lifelong learning. While research in this domain does not necessarily focus on distinguishing between synthetic and real images, the methodologies can be adapted for this purpose. For instance, Marra \etal~\cite{marra2019incremental} demonstrated how they surpassed the performance of the widely recognized continual learning method, iCaRL~\cite{rebuffi2017icarl}, by tailoring it to distinguish between real images and variations of GANs through some modifications. Their paper elaborates on how neural networks were incrementally trained with 3,600 images for each new generator introduced to the model, while preserving a fraction of the data from the seen generators for future updates. Kim \etal~\cite{kim2021cored} proposed a continual learning approach, leveraging representation learning and knowledge distillation, to adapt to new data distributions of generated images. Their study reports results across different generator families. In their setting, they used over 13,000 image samples from unseen generators while retaining a small portion of images from previously encountered generators for training. \textit{Note: Should we talk about how our method just uses 500 image samples from unseen generator here?}

%Talk about other works directly related to us, like MTMC paper. I also found this one before:  Cored: Generalizing fake media detection with continual representation using distillation. Try to find another one but it's possible that there are no others.








==> sec/background_v2.tex <==
\section{Background}

\textbf{\red{Work in Progress}}

 Since the introduction of Deep Belief Networks (DBNs) by Hinton \etal. in 2006~\cite{hinton2006fast}, generative models have undergone significant evolution, paving the way for groundbreaking developments in image generation. Variational Autoencoders (VAEs) in 2013 by Kingma and Welling~\cite{kingma2013auto}, and Generative Adversarial Networks (GANs) by Goodfellow \etal in 2014~\cite{goodfellow2014generative}, notably advanced the field, enhancing the quality and realism of synthetic images. Innovations such as Conditional GAN, CycleGAN, StyleGAN, Pix2Pix, and BigGAN further diversified applications and improved image fidelity~\cite{brock2018large,mirza2014conditional,zhu2017unpaired,isola2017image,karras2019style}. The breakthrough of diffusion models by Sohl-Dickstein \etal~\cite{sohl2015deep}, using stochastic processes for image creation, set new benchmarks in the generative landscape, significantly refined by Ho \etal in 2020~\cite{ ho2020denoising}. Presently, models like Latent Diffusion, Stable Diffusion, DALL·E, and Midjourney are generating highly detailed and imaginative visuals from various inputs, illustrating the generative models' expansive capabilities~\cite{rombach2022high,ramesh2021zero,zhang2023adding}. This progression reflects the field’s advancement towards creating synthetic imagery that closely mirrors real-life complexity, showcasing unprecedented artificial creativity and realism.
 

\subheader{Synthetic Image Detection}
%Talk about a couple of papers (Detecting and simulating artifacts in gan fake images, cnn generated images are easy to spot, Deep Image Fingerprint:
%Towards Low Budget Synthetic Image Detection and Model Lineage Analysis, etc.)
Numerous efforts have been undertaken to distinguish synthetic images from real ones. Marra \etal~\cite{marra2019gans} demonstrated that GAN-generated images possess unique 'fingerprints' useful for forensic analysis, including source identification and distinguishing between real and synthetic imagery. Zhang \etal~\cite{zhang2019detecting} introduced AutoGAN, which excels in detecting fake images without needing examples from specific GANs. Wang \etal~\cite{wang2020cnn} showed that rigorously fine-tuned with pre- and post-processing techniques and data augmentation can effectively generalize to detect CNN-based synthetic images across various generators. Most recently, Sinitsa and Fried~\cite{sinitsa2024deep} proposed DIF, a detection method using CNN architecture to identify synthetic images from GANs and diffusion model-based LTIMs, highlighting ongoing progress in synthetic image detection.

\subheader{Synthetic Image Forensic Traces}
%Talk about how forensic traces left by different generators are distinct, you can cite this paper: On the detection of synthetic images generated by diffusion models, also I think it's useful to look at their background section. Also, Learning and analyzing gan fingerprints.
Synthetic image forensic traces refer to the distinct, identifiable patterns, artifacts, or signatures left in images generated by synthetic image creation methods. It has been shown by numerous studies that every technique employed to generate synthetic visual content introduces specific traces into the resulting images, which are linked to the steps involved in the creation process~\cite{corvi2023detection, marra2019gans, yu2019attributing}. Prior works have also shown that different generator families leave significantly distinct forensic traces. This emphasizes the challenge in developing detection methods capable of generalizing across types, especially highlighting the inadequacy of knowledge transferability in synthetic image detection models~\cite{corvi2023detection}.


\subheader{Continual Learning For Synthetic Image Detection}
%Talk about continual learning, different general continual learning methods and that we can apply them to our problem and how?
Given the distinct forensic traces left by various generator families, it is crucial for image detectors to continually update their knowledge with new generators. Traditional retraining methods become impractical due to the growing number of images. An alternative is fine-tuning with images from new, unknown models, but this raises the issue of catastrophic forgetting, where neural networks lose performance on previous tasks when learning new data distributions \cite{mccloskey1989catastrophic, mcclelland1995there}. To combat this, researchers have explored continual learning approaches, which allow models to adapt without losing prior knowledge. Marra \etal~\cite{marra2019incremental} and Kim \etal~\cite{kim2021cored} have successfully applied such strategies to synthetic image detection, showing improved performance by incorporating images from both new and previously seen generators, thus demonstrating the feasibility and effectiveness of continual learning in this domain.

%Talk about other works directly related to us, like MTMC paper. I also found this one before:  Cored: Generalizing fake media detection with continual representation using distillation. Try to find another one but it's possible that there are no others.








==> sec/conclusion_v0.tex <==
\section{Conclusion}
\label{sec:conclusion}

%%% Auto generated by ChatGPT
\TODO{revise. }
In this paper, we introduce \algname, a method designed to continuously adapt to new synthetic image generators. Our approach separates the detection process into a series of expert embedders, each focused on a specific generator, and a fusion network that combines their insights. This structure directly addresses the issues of catastrophic forgetting and limited data for new generators. The key novelty lies in the method's ability to quickly adapt to new generators without losing performance on older ones. \algname offers a practical and scalable solution for the ongoing challenge of detecting images from ever-evolving synthetic image generators.



==> sec/datasets_v0.tex <==
\section{Datasets}
\label{sec:datasets}

\subsection{Baseline Dataset}
\label{subsec:baseline_ds}
We trained and evaluated our baseline synthetic image detectors on a set of publicly available datasets.
%
To form a diverse set of real images, we combined real images from the CoCo dataset~\cite{coco}, the LSUN dataset~\cite{lsun} , and the CelebA dataset~\cite{celeba}.
%
As for the set of synthetic images, we gathered GAN-generated images from the datasets used in \cite{openset, efros-easy}. 
%
These datasets are consisted of synthetic images from three different GANs: StyleGAN~\cite{stylegan}, StyleGAN2~\cite{stylegan2}, and ProGAN~\cite{progan}.
%
To form the set of images used for training, validation, and testing, we split the set of real images and the set of synthetic images each into their own disjoint sets.
%
More details are provided in Tab.~\ref{} or in the supplementary materials.
%The mentioned real datasets and GANs are commonly used to train and evaluate synthetic image generators as well as synthetic image detectors/classifiers \cite{efros-easy, luisa-diff, stylegan, stylegan2}. More details about $D_B$ are provided in \TODO{Tab \ref{tab:D_B}}. \textbf{Comment: we can put all the numbers and any other information about the dataset in the table}

\subsection{Incremental Learning Dataset}
\label{subsec:dataset_cl}
%To simulate a constantly evolving environment in which new synthetic image generators rapidly emerge, we created a dataset suitable for incremental learning setting.
To train and evaluate synthetic detection systems in the incremental learning setting, we gathered synthetic images from 20 different generators, such as Latent Diffusion~\citethis, Stable Diffusion~\citethis, StyleGAN3, Projected GAN~\citethis, \etc.
%
We refer to these generators as $G_i$, where $G_i \in \mathbb{G}$, $\mathbb{G} = \{ G_1, G_2, \cdots, G_{20} \}$. 
%
We note that these synthetic images are obtained from 3 publicly available datasets~\cite{openset,artifact,DIF}.
%
Furthermore, we denote the set of real images used in this dataset as $D^N_{real}$, which is just a subset $D^B_{real}$ and the set of data generated by $G_i$ as $D^N_{G_i}$. However, for conciseness, we will refer to $D^N_{real} \cup D^N_{G_i}$ as just $D^N_{G_i}$.
%

%
Finally, we included the set of real images from the baseline dataset described above.
%
More information about this dataset can be found in Tab. \ref{tab:incremental_ds}.


%The dataset is split into 20 sequences each associated with a different generator, which our method aims to adapt to. Each sequence of data consists of 500 real images, $D_{N_{real}}$, and 500 images synthesized by one of the generators in $D^N_{syn}$. We refer to the synthetic subset of each sequence as $D_{N_{G}}$, where $G$ could be any of the generators listed in \TODO{Tab. \ref{tab:D_N}}. \textbf{Question: Which notation to use?} We emphasize that real images are the same for all sequences; this choice has deliberately been made to evaluate our method's ability to work in scenarios where storing very small amounts of data is preferred. 



==> sec/datasets_v1_Tai.tex <==



\subheader{Baseline Detector Dataset}
We created a baseline dataset in order to train and evaluate the baseline synthetic image detectors.
%
To form a diverse set of real images, we gathered 72,000 images equally distributed among the CoCo dataset~\cite{coco}, the LSUN dataset~\cite{lsun}, and the CelebA dataset~\cite{celeba}. 
%
As for the set of synthetic images, we also gathered 72,000 GAN-generated images from the datasets used in \cite{openset, efros-easy}. 
%
The synthetic images in this set were made using 3 GANs: StyleGAN~\cite{stylegan}, StyleGAN2~\cite{stylegan2}, and ProGAN~\cite{progan}. We included the same amount of images from each of these generator in our dataset.
%
Additionally, to form the set of images used for training, validation, and testing, we split the set of real images and the set of synthetic images each into their own disjoint subsets. Specifically, we used 
120,000 images for training with 12,000 images held out for validation, and 12,000 images in a separated set for testing.
%
%The mentioned real datasets and GANs are commonly used to train and evaluate synthetic image generators as well as synthetic image detectors/classifiers \cite{efros-easy, luisa-diff, stylegan, stylegan2}. More details about $D_B$ are provided in \TODO{Tab \ref{tab:D_B}}. \textbf{Comment: we can put all the numbers and any other information about the dataset in the table}

\subheader{Emerging Generators Dataset}\label{subhead:emerging_gen_dataset}
%To simulate a constantly evolving environment in which new synthetic image generators rapidly emerge, we created a dataset suitable for incremental learning setting.
We also created an additional dataset for training and evaluating our proposed approach on detecting synthetic images made from emerging generators in a continual learning setting. 
%
To accomplish this, we first selected a comprehensive and diverse set of generators, composed of 19 different generation techniques. These techniques are listed in Tab.~\ref{tab:gen_abv}. All synthetic images in this dataset are assembled from publicly available datasets~\cite{openset,artifact,DIF}.
Then, to update our and others' baseline detectors, we used a set of 500 images from each generator. And we used a disjoint set of 400 images from each generator to evaluate the performance of all detectors.


%The dataset is split into 20 sequences each associated with a different generator, which our method aims to adapt to. Each sequence of data consists of 500 real images, $D_{N_{real}}$, and 500 images synthesized by one of the generators in $D^N_{syn}$. We refer to the synthetic subset of each sequence as $D_{N_{G}}$, where $G$ could be any of the generators listed in \TODO{Tab. \ref{tab:D_N}}. \textbf{Question: Which notation to use?} We emphasize that real images are the same for all sequences; this choice has deliberately been made to evaluate our method's ability to work in scenarios where storing very small amounts of data is preferred. 



==> sec/datasets_v2_Aref.tex <==



\subheader{Baseline Detector Dataset}
We created a baseline dataset in order to train and evaluate the baseline synthetic image detectors.
%
To form a diverse set of real images, we gathered 72,000 images equally distributed among the CoCo dataset~\cite{coco}, the LSUN dataset~\cite{lsun}, and the CelebA dataset~\cite{celeba}. 
%
As for the set of synthetic images, we also gathered 72,000 GAN-generated images from the datasets used in \cite{openset, efros-easy}. 
%
The synthetic images in this set were made using three GANs: StyleGAN~\cite{stylegan}, StyleGAN 2~\cite{stylegan2}, and ProGAN~\cite{progan}. We included 24,000 images from each of these generators in our dataset.
%
Additionally, to form the set of images used for training, validation, and testing, we split the set of real images and the set of synthetic images each into their own disjoint subsets. Specifically, we used 
132,000 images for training with 12,000 images held out for validation, and 12,000 images in a separate set for evaluation.
%
%The mentioned real datasets and GANs are commonly used to train and evaluate synthetic image generators as well as synthetic image detectors/classifiers \cite{efros-easy, luisa-diff, stylegan, stylegan2}. More details about $D_B$ are provided in \TODO{Tab \ref{tab:D_B}}. \textbf{Comment: we can put all the numbers and any other information about the dataset in the table}

\subheader{Emerging Generators Dataset}\label{subhead:emerging_gen_dataset}
To simulate a constantly evolving environment in which new synthetic image generators rapidly emerge, we created a dataset to train and evaluate our proposed approach in a continual learning setting.
% We also created an additional dataset for training and evaluating our proposed approach on detecting synthetic images made from emerging generators in a continual learning setting. 
%
To accomplish this, we first selected a diverse set of generators, composed of 19 different generation techniques. These techniques are listed in Tab.~\ref{tab:gen_abv}. All synthetic images in this dataset are assembled from publicly available datasets~\cite{openset,artifact,DIF}.
Next, to update baseline detectors using our and competing approaches, we used a set of 500 images from each generator. We then used a disjoint set of 400 images from each generator to evaluate the performance of all detectors.


%The dataset is split into 20 sequences each associated with a different generator, which our method aims to adapt to. Each sequence of data consists of 500 real images, $D_{N_{real}}$, and 500 images synthesized by one of the generators in $D^N_{syn}$. We refer to the synthetic subset of each sequence as $D_{N_{G}}$, where $G$ could be any of the generators listed in \TODO{Tab. \ref{tab:D_N}}. \textbf{Question: Which notation to use?} We emphasize that real images are the same for all sequences; this choice has deliberately been made to evaluate our method's ability to work in scenarios where storing very small amounts of data is preferred. 



==> sec/discussion_v0.tex <==
\section{Discussion}
\label{sec:discussion}

Our method's high performance can be attributed to the fact that we train dedicated sub-networks for each new generator.  These sub-networks act as an expert capable of mapping an image from a new generator to an embedding space specifically learned for that generator's data. In one embedding space, classifying real images and images synthesized by the associated generator should be fairly straightforward. Additionally, the transformer help the classification layer by highlighting the relevant and de-emphasizing less relevant information.

This approach comes with a cost of growing the network size whenever a new generator appears. However, there is an intrinsic trade-off between the error rate and the network size. Although the network size grows linearly with the number of added generators, the performance gain over existing methods is substantial. On top of that, we could run all of our experiments on a machine with a single NVIDIA RTX 3090 GPU, which is quite affordable. 

%

Additionally, as shown in Fig.~\ref{fig:exp3}, our method is capable of achieving impressively high performance given even more limited amounts of data from the new generators. We note that with having access to only \red{???} number of images, our method still outperforms UDIL with access to 500 images.

==> sec/discussion_v1_Aref.tex <==
\section{Discussion}
\label{sec:discussion}

Our method's high performance can be attributed to the fact that it utilizes dedicated embedders for each new generator.  These sub-networks act as experts capable of mapping images from a new generator to an embedding space specifically learned for that generator. In a specialized embedding space, classifying real images and images synthesized by the associated generator is fairly straightforward . Therefore, by utilizing an ensemble of expert embedders, and subsequently fusing their knowledge, our method is capable of reliably detecting synthetic images from new generators without forgetting identifying the old ones. 

This approach comes with a cost of growing the network size whenever a new generator appears. However, there exists an intrinsic trade-off between the error rate and the network size. Although the network size grows linearly with the number of added generators, the performance gain over existing methods is substantial. It is noteworthy to mention that we could run all of our method's experiments on a machine with a single NVIDIA RTX 3090 GPU.

%
Additionally, as shown in Fig.~\ref{fig:effects_new_gen_data_size}, our method is capable of achieving impressively high performance given even more limited amounts of data from each new generator. The results show that even with having access to an order of magnitude lower amounts of training images per generator, our method can still outperforms all other competing methods.

==> sec/discussion_v2_Aref.tex <==
\section{Discussion}
\label{sec:discussion}

Our method's impressive performance can be attributed to its utilization of dedicated embedders for each new generator. These embeddings are specifically learned to capture forensic traces left by their corresponding generators. As a result, our algorithm does not rely solely on a single embedding space, but rather the union of all embedding spaces from every expert embedder.

However, our approach does come at a cost of increased the network size. 
% The size of the whole network grows linearly for each new generator being introduced. 
Despite this, the cost of mis-detecting AI-generated images, or false-alarming real images as being synthetic, is worth the increase in network parameters. Additionally, it's important to note that after our method adapted the baseline detector based on MISLnet to 19 different generators, the total number of parameters in our network is 27.8M parameters. However, 25.1M of these parameters are frozen because they come from the set of ensemble of embedders. In reality, at each introduction of a new generator, we only train the new expert embedder along with the EFKN, which in total is only a constant of about 4M parameters. To put this into context, after adding 100 new generators, the trainable portion of our network is only 13.6M parameters, a number smaller than a single ResNet-50 model of 23.5M parameters.





==> sec/exp1_add_single_gen_v0.tex <==
\subsection{Adding a Single New Generator}
\label{subsec:exp1_add_single_gen}



\input{tables/exp1.tex}
In this set of experiments, we evaluated our method and the competing methods' ability to update a baseline detector to detect images from a single new generator. To do that, we separately updated the baseline detectors using our approach and all the competing methods. Next, we repeated the same experiment for all of the 19 generators listed in Tab~\ref{tab:gens_ds}.
We then measured the performance in terms of AUC score with 50\% of synthetic images being from the baseline dataset and the rest of synthetic images generated by the new generator. We also calculated and reported the average AUC across all generators for each method. Finally, we calculated our method's Relative Error Reduction (RER) in terms AUC with respect to the competing methods.
%
In these experiments, we used a memory of size 1000 images equally divided between real and synthetic from the baseline dataset. Additionally, each update technique had access to 500 training images from the new generator. 
%



Tab.~\ref{tab:exp1} shows the results of this series of experiments. These findings demonstrate that our method is capable of extracting traces specific to new generators and successfully train a classifier to detect the images from both the previously seen and the new generators. Our approach achieves a final average AUC score of 0.99 across all generators significantly higher compared to the competing methods.
%
Specifically, our method gains an RER of {66\%} over the second best method, \ie UDIL.
%

Different generators enforce different levels of adaptation complexity to the update methods, which tends to be a result of the baseline detector failing to completely transfer its knowledge to images from those generators.
Nonetheless, even in the most challenging cases, \eg, Latent Diffusion, our approach still significantly outperforms the rest and achieves an AUC score of 0.96 with an RER of 55\% over UDIL.
%
Moreover, our method's performance on different generators has the least variance compared to all competing methods, demonstrating stability.
%

We also observe that the baseline detector performs better than fine-tuning in many cases. Although naive fine-tuning results in high performance on detecting the new generators' data, it leads to catastrophic forgetting, which results in significant performance drop on the baseline dataset.
The results demonstrate that our method successfully tackles the problem of learning a common embedding space where both previously seen and the new generators can be reliably separated from the real images.

==> sec/exp1_add_single_gen_v1_Tai.tex <==
\subsection{Adapting to One Emerging Generator}
\label{subsec:exp1_add_single_gen}

\input{tables/exp1.tex}

In this experiment, we evaluated our approach's ability to detect synthetic images from a single emerging generator. We then compared our method's performance to other techniques used to update the baseline detector. We note that all approaches started with the same baseline detector network. We repeated this experiment with all available generators in the set of emerging generators listed in Tab.~\TODO{refer}. We presented the results of these experiments in Tab.~\ref{tab:exp1}, where each column's number is the performance of an algorithm adapting from the baseline to a specific generator, and the final column represents the average over all generators.


\begin{comment}

In this set of experiments, we evaluated our method and the competing methods' ability to update a baseline detector to detect images from a single new generator. To do that, we separately updated the baseline detectors using our approach and all the competing methods. Next, we repeated the same experiment for all of the 19 generators listed in Tab~\ref{tab:gens_ds}.
We then measured the performance in terms of AUC score with 50\% of synthetic images being from the baseline dataset and the rest of synthetic images generated by the new generator. We also calculated and reported the average AUC across all generators for each method. Finally, we calculated our method's Relative Error Reduction (RER) in terms AUC with respect to the competing methods.
%
In these experiments, we used a memory of size 1000 images equally divided between real and synthetic from the baseline dataset. Additionally, each update technique had access to 500 training images from the new generator. 
%
\end{comment}


The results of our experiment in Tab.~\ref{tab:exp1}
show that our method achieves the best detection performance across each and every emerging generator with the average AUC of 0.99. 
%
Additionally, it can be observed that our approach consistently obtained strong performance (0.96 AUC or above) no matter what generator it adapted to. 
%
Notably, the second best method, UDIL, obtained an average AUC of 0.97. However, our method's performance of 0.99 AUC is a significant 66\% decrease in Relative Error Reduction (RER\%) compared to UDIL.

These results show that our method, which involves developing a specialized expert detector for the emerging generator and integrating knowledge from both new and existing experts, is an effective technique to adapt to a new emerging synthetic generator. 
Furthermore, our method outperforms competing strategies that rely on continuously adjusting the network weights of the baseline detector. This phenomenon is likely due to the fact that our approach is not restricted to operate on a set of features from a single embedding space, but rather a much broader set of features resulted from aggregating multiple embedding spaces.

It is also noteworthy that the baseline detector, without seeing the new generator, outperforms the naive fine-tuning method on multiple instances. This is because while the fine-tuned detectors performs well on the new generator, it forgets most of what it had learned for the baseline generators. This result shows the direct effect of catastrophic forgetting which aligns with findings from prior works~\citethis.


\begin{comment}
    

is capable of extracting traces specific to new generators and successfully train a classifier to detect the images from both the previously seen and the new generators. Our approach achieves a final average AUC score of 0.99 across all generators significantly higher compared to the competing methods.
%
Specifically, our method gains an RER of {} over the second best method, \ie UDIL.
%

Different generators enforce different levels of adaptation complexity to the update methods, which tends to be a result of the baseline detector failing to completely transfer its knowledge to images from those generators.
Nonetheless, even in the most challenging cases, \eg, Latent Diffusion, our approach still significantly outperforms the rest and achieves an AUC score of 0.96 with an RER of 55\% over UDIL.
%
Moreover, our method's performance on different generators has the least variance compared to all competing methods, demonstrating stability.
%

We also observe that the baseline detector performs better than fine-tuning in many cases. Although naive fine-tuning results in high performance on detecting the new generators' data, it leads to catastrophic forgetting, which results in significant performance drop on the baseline dataset.
The results demonstrate that our method successfully tackles the problem of learning a common embedding space where both previously seen and the new generators can be reliably separated from the real images.

\end{comment}

==> sec/exp1_add_single_gen_v2_Tai.tex <==

\subsection{Adapting to A Single New Generator}
\label{subsec:exp1_add_single_gen}



In this experiment, we evaluated our approach's ability to detect synthetic images from a single new generator. We then compared our method's performance to other techniques used to update the baseline detector. We note that all approaches started with the same baseline detector network. Subsequently, we repeated this experiment with all available generators in the set of emerging generators listed in Tab.~\ref{tab:gen_abv}. We presented the results of these experiments in Tab.~\ref{tab:exp1_add_single_new_gen}. In this table, each column represents the performance of different algorithms adapting the baseline detector to the specific generator. The final column represents the average and the standard deviation calculated for each algorithm over the whole set of new generators.

% , where in each column the numbers are the performance of an algorithm adapting from the baseline to a specific generator, and the final column represents the average over all generators.


The results of our experiment in Tab.~\ref{tab:exp1_add_single_new_gen}
show that our method achieves the best detection performance across all possible new generators with an average AUC of 0.99. Effectively, our method gains a significant relative error reduction of 66\% over the second best performing method, UDIL. 

%The second best method is UDIL~\cite{udil}, whose average AUC is 0.97. This means that our method gains an RER of 66\% over UDIL in terms of AUC.

Additionally, we observed that our approach consistently obtained a strong performance of 0.96 AUC or above with a standard deviation of only 0.01 AUC. In contrast, other competing methods' performance has standard deviations of about 3 to 10 times larger. This demonstrates the fact that our EEE, irrespective of the new generator added, is the most stable among all methods 

%This demonstrat that irrespective of the new generator, our approach is well equipped to detect its generated images.

Furthermore, it is important to highlight that on some occasions when the baseline detector experiences a significant performance drop detecting a specific unseen generator, other approaches also tend to exhibit a similar drop in performance. For example, all competing methods have a significant drop adapting to Latent Diffusion (LD) and BigGAN (BG). Similarly, LWF has difficulties with DLM, DER++, MT-SC and MT-MC with SD1.1, SD1.4 \& SD2.1, and ICaRL with SD1.1 \& SD1.4. This result is un-surprising, however, because the baseline detectors were trained on GANs so adapting to Diffusion-based generators is much more challenging, as shown in prior work~\cite{corvi2023detection}.

In contrast, our approach displays stable performance no matter which generator were added. This is likely due to the fact that we produced a dedicated expert embedder for the new generator instead of updating our baseline detector, like other approaches. By doing this, we don't have to rely on learning a single embedding space to capture traces of both existing generators and the new generator. This is particularly true when the new generator's forensic traces are distinct from those previously learned. 




\begin{comment}

Notably, the second best method, UDIL, obtained an average AUC of 0.97. However, our method's performance of 0.99 AUC is .

These results show that our method, which involves developing a specialized expert detector for the emerging generator and integrating knowledge from both new and existing experts, is an effective technique to adapt to a new emerging synthetic generator. 
Furthermore, our method outperforms competing strategies that rely on continuously adjusting the network weights of the baseline detector. This phenomenon is likely due to the fact that our approach is not restricted to operate on a set of features from a single embedding space, but rather a much broader set of features resulted from aggregating multiple embedding spaces.

It is also noteworthy that the baseline detector, without seeing the new generator, outperforms the naive fine-tuning method on multiple instances. This is because while the fine-tuned detectors performs well on the new generator, it forgets most of what it had learned for the baseline generators. This result shows the direct effect of catastrophic forgetting which aligns with findings from prior works~\citethis.

\end{comment}

==> sec/exp1_add_single_gen_v3_Aref.tex <==

\subsection{Adapting to A Single New Generator}
\label{subsec:exp1_add_single_gen}



In this experiment, we evaluated our approach's ability to detect synthetic images from a single new generator. We then compared our method's performance to other techniques used to update the baseline detector. We note that all approaches started with the same baseline detector network. Subsequently, we repeated this experiment with all available generators in the set of emerging generators listed in Tab.~\ref{tab:gen_abv}. We presented the results of these experiments in Tab.~\ref{tab:exp1_add_single_new_gen}. In this table, each column represents the performance of different algorithms adapting the baseline detector to the specific generator. The final column represents the average and the standard deviation calculated for each algorithm over the whole set of new generators.

% , where in each column the numbers are the performance of an algorithm adapting from the baseline to a specific generator, and the final column represents the average over all generators.


The results of our experiment in Tab.~\ref{tab:exp1_add_single_new_gen}
show that our method achieves the best detection performance across all possible new generators with an average AUC of 0.99. Effectively, our method gains a significant relative error reduction of 66\% over the second best performing method, UDIL. 

%The second best method is UDIL~\cite{udil}, whose average AUC is 0.97. This means that our method gains an RER of 66\% over UDIL in terms of AUC.

Additionally, we observed that our approach consistently obtained a strong performance of 0.96 AUC or above with a standard deviation of only 0.01 AUC. In contrast, other competing methods' performance has standard deviations of about 3 to 10 times larger. This demonstrates that irrespective of the synthetic images' underlying generation method, our approach is well-equipped to detect them.

%This demonstrat that irrespective of the new generator, our approach is well equipped to detect its generated images.

Furthermore, it is important to highlight that on some occasions when the baseline detector experiences a significant performance drop detecting a specific unseen generator, other approaches also tend to exhibit a similar drop in performance. For example, all competing methods have a significant drop adapting to Latent Diffusion (LD) and BigGAN (BG). Similarly, LWF has difficulties with DLM, DER++, MT-SC and MT-MC with SD1.1, SD1.4 \& SD2.1, and ICaRL with SD1.1 \& SD1.4. This result is un-surprising, however, because the baseline detectors were trained on GANs. Therefore, as shown in prior work~\cite{corvi2023detection}, adapting to diffusion-based generators is more challenging.

In contrast, our approach displays stable performance irrespective of which generator were added. This is likely due to the fact that our approach is not restricted to operate on a single embedding space, but rather a comprehensive set of embeddings resulted from aggregating multiple embedding spaces. By doing this, we do not need to rely on learning a single embedding space to capture traces of both existing and the new generators. 

%This is particularly true when the new generator's forensic traces are distinct from those previously learned. 

\begin{comment}

Notably, the second best method, UDIL, obtained an average AUC of 0.97. However, our method's performance of 0.99 AUC is .

These results show that our method, which involves developing a specialized expert detector for the emerging generator and integrating knowledge from both new and existing experts, is an effective technique to adapt to a new emerging synthetic generator. 
Furthermore, our method outperforms competing strategies that rely on continuously adjusting the network weights of the baseline detector. This phenomenon is likely due to the fact that our approach is not restricted to operate on a set of features from a single embedding space, but rather a much broader set of features resulted from aggregating multiple embedding spaces.

It is also noteworthy that the baseline detector, without seeing the new generator, outperforms the naive fine-tuning method on multiple instances. This is because while the fine-tuned detectors performs well on the new generator, it forgets most of what it had learned for the baseline generators. This result shows the direct effect of catastrophic forgetting which aligns with findings from prior works~\citethis.

\end{comment}

==> sec/exp1_add_single_gen_v4_Tai.tex <==

\subsection{Adapting to One New Generator}
\label{subsec:exp1_add_single_gen}



In this experiment, we evaluated our approach's ability to detect synthetic images from one new generator. We repeated this experiment for all 19 generators in our dataset. This is important because in reality we do not know beforehand which generator we need to adapt our detector to. 
We then compared our method's performance to other techniques used to update the baseline detector. We note that all approaches started with the same baseline detector network. 

We presented the results of these experiments in Tab.~\ref{tab:exp1_add_single_new_gen}. In this table, each column represents the performance of different algorithms adapting the baseline detector to the specific generator. The final column represents the average and the standard deviation calculated for each algorithm over the whole set of new generators.

% , where in each column the numbers are the performance of an algorithm adapting from the baseline to a specific generator, and the final column represents the average over all generators.


The results of our experiment in Tab.~\ref{tab:exp1_add_single_new_gen}
show that our method achieves the best detection performance across all possible new generators with an average AUC of 0.99. Compared to the second best method, UDIL, whose an average AUC is 0.97, we obtained a significant relative error reduction of 66\%. This shows that our approach is able to learn a more effective set of features than other competing methods. This effect is likely caused by the fact that our approach can operate on a more inclusive embedding space, while others are restricted to adapting a single embedding space.

Additionally, we note that other competing methods' performance has standard deviations of about 3 to 10 times larger than ours. This result can be further examined by looking at certain occasions when the baseline detector experiences a significant performance drop detecting a specific unseen generator. When this happens, other approaches also tend to exhibit a similar drop in performance. For example, all competing methods have a significant drop adapting to Latent Diffusion (LD) and BigGAN (BG). Similarly, LWF has difficulties with DLM, DER++, MT-SC and MT-MC with SD1.1, SD1.4 \& SD2.1, and ICaRL with SD1.1 \& SD1.4. This result is not surprising, however, because the baseline detectors were trained on GANs. Therefore, as shown in prior work~\cite{corvi2023detection}, adapting to diffusion-based generators is more challenging.

In contrast, our approach displays stable performance irrespective of which generator were added. This is likely due to the fact that our approach does not need to rely heavily on learning a single embedding space to capture traces of both existing and the new generators. 

%This is particularly true when the new generator's forensic traces are distinct from those previously learned. 

\begin{comment}

Notably, the second best method, UDIL, obtained an average AUC of 0.97. However, our method's performance of 0.99 AUC is .

These results show that our method, which involves developing a specialized expert detector for the emerging generator and integrating knowledge from both new and existing experts, is an effective technique to adapt to a new emerging synthetic generator. 
Furthermore, our method outperforms competing strategies that rely on continuously adjusting the network weights of the baseline detector. This phenomenon is likely due to the fact that our approach is not restricted to operate on a set of features from a single embedding space, but rather a much broader set of features resulted from aggregating multiple embedding spaces.

It is also noteworthy that the baseline detector, without seeing the new generator, outperforms the naive fine-tuning method on multiple instances. This is because while the fine-tuned detectors performs well on the new generator, it forgets most of what it had learned for the baseline generators. This result shows the direct effect of catastrophic forgetting which aligns with findings from prior works~\citethis.

\end{comment}

==> sec/exp2_add_multi_gen_v0.tex <==
\subsection{Adapting to Multiple Emerging Generator}
\label{subsec:exp2_add_multi_gen}



\input{tables/exp2.tex}
Here, we compare our method and the competing methods' capability to adapt a baseline detector to a series of new generators. In this experiment, we used the update methods to sequentially update the baseline detectors using all sets of data available in the new generator dataset. Each method had access to a buffer of 1000 images equally divided between real and synthetic images. To ensure fairness for all generators, we used a random uniform sampling strategy to select the 500 synthetic images from the already observed generators.
%
After each episode, we measured the models' performance in terms of average AUC over the test sets associated with the current and the previous generators. The test data of each step consisted of a common set of 400 real images and 400 synthetic images associated with the new generator. 
We also measured our method's RER with respect to all the competing methods.

%

The results of this experiment is provided in Tab.~\ref{tab:exp2}. Our method demonstrates advantageous performance by achieving a final average AUC of 0.97, significantly higher than all other methods. Notably, our approach gains an RER of 57\% over the second best method, \ie UDIL. Additionally, our method shows consistently higher performance irrespective of the new generator over all other methods. This shows that our approach can learn traces of new generators while maintaining its performance on the previous ones, even when adding a large number of generators.
%

We also note that applying our method results in a performance loss as small as only 0.02 AUC compared to the baseline performance. Other methods, on the other hand, suffer dramatically after encountering new sources of synthetic image. Specifically, UDIL's performance loss is 200\% more than that of our method (\red{is this the correct way to say it? 0.02 vs 0.06}). The trend of performance loss suggests that our method can face even comparatively less performance loss when more and more generators are introduced to the system.

==> sec/exp2_add_multi_gen_v1_Tai.tex <==
\subsection{Adapting to Multiple Emerging Generator}
\label{subsec:exp2_add_multi_gen}


In this experiment, we evaluate our approach's ability to adapt to multiple sequentially emerging generators. We then compared our method's performance to other dedicated continual learning techniques. All methods started with the same baseline detector network. 
% While our approach continuously produced new expert detectors for each emerging generators and fused their knowledge using the \reasoner, others methods performed an update to the same, previously trained detector at each emergence. 
After adapting to detect synthetic images from a new generator, we measured our and competing methods' performance in terms of average AUC over the test sets associated with the current and the previous generators. 
% The test data of each step consisted of a common set of 400 real images and 400 synthetic images associated with the emerging generator. 
We presented the results of this experiment in Tab.~\ref{tab:exp2_add_multi_new_gen}.

Results in Tab.~\ref{tab:exp2_add_multi_new_gen} show that our approach achieved the best performance irrespective of the number of new generators added.
Furthermore, we observed that after continually adapting to 19 different generators, our method obtained an average AUC of 0.97, a reduction of only 0.02 when compared to the initial performance of 0.99 average AUC. This result is a significant improvement over the second best method, UDIL, with 0.93 AUC. 
Additionally, it can be seen from Tab.~\ref{tab:exp2_add_multi_new_gen} that the more the number of new generators is introduced, the more degraded the performance of some competing approaches (\ie LWF, DER++, MT-SC). However, our method retained strong performance throughout our experiment, with minimal reduction in performance.

Additionally, We note that other competing methods all experience difficulties detecting new synthetic images from some particular generator. For example, LWF \& ER experienced significant performance drop when adapting to DALL-E 2 (DL2), similarly, UDIL's performance dropped adapting to BigGAN (BG), and ICaRL's, MT-SC's, MT-MC's are performance substantially lower adapting to Latent Diffusion (LD). However, our proposed approach does not experience such issues. Our results show that by fusing the knowledge of all past and current experts, we can gracefully adapt to any new generator while avoid having significant performance degradation as the number of generator being added increases. 


\begin{comment}

Here, we compare our method and the competing methods' capability to adapt a baseline detector to a series of new generators. In this experiment, we used the update methods to sequentially update the baseline detectors using all sets of data available in the new generator dataset. Each method had access to a buffer of 1000 images equally divided between real and synthetic images. To ensure fairness for all generators, we used a random uniform sampling strategy to select the 500 synthetic images from the already observed generators.
%
After each episode, we measured the models' performance in terms of average AUC over the test sets associated with the current and the previous generators. The test data of each step consisted of a common set of 400 real images and 400 synthetic images associated with the new generator. 
We also measured our method's RER with respect to all the competing methods.

%

Our method demonstrates advantageous performance by achieving a final average AUC of 0.97, significantly higher than all other methods. Notably, our approach gains an RER of 57\% over the second best method, \ie UDIL. Additionally, our method shows consistently higher performance irrespective of the new generator over all other methods. This shows that our approach can learn traces of new generators while maintaining its performance on the previous ones, even when adding a large number of generators.
%

We also note that applying our method results in a performance loss as small as only 0.02 AUC compared to the baseline performance. Other methods, on the other hand, suffer dramatically after encountering new sources of synthetic image. Specifically, UDIL's performance loss is 200\% more than that of our method (\red{is this the correct way to say it? 0.02 vs 0.06}). The trend of performance loss suggests that our method can face even comparatively less performance loss when more and more generators are introduced to the system.

\end{comment}













==> sec/exp3_data_size_v0.tex <==
\input{figures/effects_new_gen_data_size}

\subsection{Effects of New Generator's Training Data Size}
\label{subsec:exp3_new_gen_data_budget}

In this experiments, we examined the effects of the emerging generator's training data size on our proposed approach. To conduct this experiment, we used the same training procedure and hyper-parameters as the previous experiment in Sec.~\ref{subsec:exp2_add_multi_gen}, but we varied the amount of data, $N_2$, from each the emerging generator available to our method. In particular, we trained our experts embedders with $N_2 = \{500, 400, 300, 200, 100, 50\}$ and tested our algorithm using the same testing set as in Sec.~\ref{subsec:exp2_add_multi_gen}. We then reported the average AUC after sequentially adding all 19 generators in our dataset. The result of this experiment is shown in Fig.~\ref{fig:effects_new_gen_data_size}.


Results from Fig.~\ref{fig:effects_new_gen_data_size} show that our method experienced minimal declines in detection performance as the number of available training images decreases. Specifically, our performance at $N_2 = 500$ is 0.97 average AUC and at $N_2 = 50$ is 0.94 average AUC, resulting in only a drop of 0.042 average AUC. 
Additionally, we note that our performance at having only 50 training data sample for each new generator is 0.94 average AUC, which is an improvement over UDIL's 0.93 average AUC with 10 times the training data size. These result suggest that our approach not only achieves strong and reliable performance adapting to detect synthetic images coming from new generators, but also requires less data than other methods to obtain good performance.

==> sec/exp3_data_size_v1.tex <==
\input{figures/effects_new_gen_data_size}

\subsection{Effects of New Generator's Training Data Size}
\label{subsec:exp3_new_gen_data_budget}

In this experiment, we explored the impact of training data size from emerging generators on our proposed approach. We employed the same training procedures and hyper-parameters as in the previous experiment described in Sec 
%
\ref{subsec:exp2_add_multi_gen}, but varied the amount of data, $N_2$, from each emerging generator available to our method. Specifically, we trained our expert embedders with $N_2 = {500, 400, 300, 200, 100, 50}$ and evaluated our algorithm using the same testing set as in Sec.\ref{subsec:exp2_add_multi_gen}. We then reported the average AUC and accuracy after sequentially adding all 19 generators to our dataset. The results of this experiment are depicted in Fig.~\ref{fig:effects_new_gen_data_size}.

The results, as illustrated in Fig.~\ref{fig:effects_new_gen_data_size}, indicate that our method experienced minimal declines in detection performance as the number of available training images decreased. Specifically, our performance at $N_2 = 500$ was an average AUC of 0.97, and at $N_2 = 100$, it was 0.96, resulting in only a drop of 0.01 in average AUC. Additionally, our performance with only 50 training data samples for each new generator was an average AUC of 0.94, demonstrating an improvement over UDIL's average AUC of 0.93 with ten times the training data size. These results suggest that our approach not only achieves strong and reliable performance in adapting to detect synthetic images from new generators but also requires less data than other methods to achieve good performance.

==> sec/exp3_data_size_v2_Aref.tex <==
\subsection{Effects of New Generator's Training Data Size}
\input{figures/effects_new_gen_data_size}
\label{subsec:exp3_new_gen_data_budget}

In this experiment, we explored the impact of training data size from new generators on our proposed approach. We employed the same training procedures and hyper-parameters as in the previous experiment described in Sec~\ref{subsec:exp2_add_multi_gen}, but varied the amount of data available to our method, $N$, from each new generator. 
%
Specifically, we trained our expert embedders  with $N \in \{500, 400, 300, 200, 100, 50\}$ and evaluated our algorithm using the same testing set as in Sec.~\ref{subsec:exp2_add_multi_gen}. We then reported the average AUC and accuracy after sequentially adding all 19 generators to our dataset. The results of this experiment are depicted in Fig.~\ref{fig:effects_new_gen_data_size}.

The results in Fig.~\ref{fig:effects_new_gen_data_size} show that our method's performance experienced minimal reduction in detection performance as the number of available training images decreased. Specifically, our performance at $N = 500$ is 0.97 average AUC, and at $N = 50$ is 0.96 average AUC, resulting in a drop of only 0.01 in average AUC. Additionally, our performance of 0.94 average AUC with only 50 training data samples for each new generator is still an improvement over UDIL, whose training data size is 10 times larger than ours. These results suggest that our approach not only achieves the highest performance in adapting to detect synthetic images from new generators but also requires significantly less data than other methods to achieve strong performance.

% The results, as illustrated in Fig.~\ref{fig:effects_new_gen_data_size}, demonstrate that our method experience minimal declines in detection performance as the number of available training images decrease. Specifically, our method's performance at $N = 500$ and $N = 100$ is 0.97, and 0.96 in terms of average AUC, respectively

% is an average AUC of 0.97, and at $N = 100$, it was 0.96, resulting in only a drop of 0.01 in average AUC. Additionally, our performance with only 50 training data samples for each new generator was an average AUC of 0.94, demonstrating an improvement over UDIL's average AUC of 0.93 with ten times the training data size. These results suggest that our approach not only achieves strong and reliable performance in adapting to detect synthetic images from new generators but also requires less data than other methods to achieve good performance.

==> sec/exp3_data_size_v3_Tai.tex <==
\subsection{Effects of New Generator's Training Data Size}
\input{figures/effects_new_gen_data_size}


\label{subsec:exp3_new_gen_data_budget}


In this experiment, we examined the impact of training data size from each new generator on our proposed approach. This is important because in real world scenarios, the amount of available data from a new generator is often limited, especially if such generator is a proprietary product.
Therefore, to conduct this experiment, we repeated the experiment in Sec~\ref{subsec:exp2_add_multi_gen}, 
with different numbers of available data ranging from 50 to 500 data points. 
We then reported the average AUC and accuracy after sequentially adding all 19 generators to our dataset. Additionally, due to limit of space, we compared our approach to UDIL, the best performing method in both experiments in Sec~\ref{subsec:exp1_add_single_gen}~\&~\ref{subsec:exp2_add_multi_gen}.

The results of this experiment are depicted in Fig.~\ref{fig:effects_new_gen_data_size}.
These results show that our method's performance experienced minimal reduction in detection performance as the number of available training images decreased. Specifically, we experience a very slight drop in performance (0.97 to 0.95 average AUC) while having 5 times less training data, and a small drop in performance (0.97 to 0.94 average AUC) with 10 times less data. Notably, our performance of 0.94 average AUC is still an improvement over UDIL (0.93 AUC), whose training data size is 10 times larger than ours (see Sec.~\ref{subsec:exp2_add_multi_gen}).
These results suggest that our approach not only achieves the highest performance in adapting to detect synthetic images from new generators but also requires significantly less data than other methods to achieve strong performance.













==> sec/exp4_effects_of_diff_archs_v0.tex <==
\subsection{Effects of Different Detector Architectures}
\label{subsec:exp4_diff_arch}

In this experiment, we examined the effects of utilizing different network architectures for the underlying detector. We applied our proposed approach and UDIL's approach on 
three different network architectures: ResNet-50~\citethis, SR-Net~\citethis, and DenseNet~\citethis. These networks are widely used in prior work for synthetic image detection. For this experiment, we used the identical emerging generator's training data size and memory buffer size as our prior experiment in Sec.~\ref{subsec:exp2_add_multi_gen}. We presented this experiment's result in Tab.~\ref{tab:exp4_archs}.

The results from Tab.~\ref{tab:exp4_archs} show that our proposed approach achieved the best performance regardless of the underlying detector architecture. 
In particular, \TODO{fill this in when results are in}



==> sec/exp4_effects_of_diff_archs_v1_Aref.tex <==
\subsection{Effects of Different Detector Architectures}
\label{subsec:exp4_diff_arch}

\input{tables/exp4_different_archs}

In this experiment, we examined the effects of utilizing different network architectures for the baseline detector. We applied our method, EEE, and UDIL on
three different network architectures: ResNet-50~\cite{resnet}, SR-Net~\citethis, and DenseNet~\citethis. These networks are widely used in prior work for synthetic image detection. For this experiment, we used the identical emerging generator's training data size, $N$ and memory buffer size, $M$ as our prior experiment in Sec.~\ref{subsec:exp2_add_multi_gen}. We presented this experiment's results in Tab.~\ref{tab:exp4_archs}.

The results from Tab.~\ref{tab:exp4_archs} show that our proposed approach achieved the best performance regardless of the underlying detector architecture. 
In particular, \TODO{fill this in when results are in}



==> sec/exp_setup_v1.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{subsec:exp_setup}

We ran a series of experiments to demonstrate our method's ability to adapt a baseline detector to be able to detect images from a new synthetic image generator. Basic experimental procedures are described below.

\subheader{Baseline Detectors} 
To train our baseline detectors we use two different architectures: ResNet50~\cite{resnet} which is widely used for synthetic image detection~\citethis, and MISLnet~\cite{mislnet} which is used for forensic manipulation detection~\citethis. These networks are trained via the ADAM optimizer~\citethis with the default hyper-parameters on randomly selected patches of size 256 $\times$ 256 obtained from the baseline training dataset. 
%
The ResNet50 is trained with an initial learning rate of $1.0 \times 10^{-4}$, which is further decayed by a factor of $0.75$ every 3 epochs. 
This model has an accuracy of 0.95 and an area under the ROC curve (AUC) of 0.99 on the baseline test dataset.
%
The MISLnet, on the other hand, is trained with a constant learning rate of $5.0 \times 10^{-5}$, and achieves an accuracy of 0.97 and an AUC of 0.99.
We note that during validation and testing phase, we extract patches from the center of the images.


\subheader{Competing Methods}
We compared our method against multiple competing approaches appropriate for our problem setting. 
%
First, we included a naive approach, which is simply fine-tuning the baseline detectors on the data generated by each new generator. Additionally, we compared against well-established and state-of-the-art continual learning methods, such as Learning Without Forgetting (LWF)~\citethis, Experience Replay (ER)~\citethis, ICaRL~\citethis, and Unified Domain Incremental Learning (UDIL)~\cite{udil}. It is noteworthy that UDIL has specifically been designed for continual learning scenarios where the continual learner is expected to adapt to new domains of data, without introducing any new classes. This is quite similar to our problem setting. The rest of continual learning methods techniques could readily or with slight modifications be applied to our problem. We implemented ICaRL ourselves and used the implementations provided by~\cite{udil} for the rest of the continual learning methods.
%

We also implemented two methods introduced by Marra \etal~\citethis, which specifically were developed to update synthetic image detectors with the data synthesized by new generators, and compared against them. Lastly, we included the baseline detectors performance on the new synthetic images as a lower-bound. These models did not undergo any updates with new generators data and solely rely on transferability.




































\begin{comment}
\begin{equation}
	\small
	\label{eq:rer}
	100 \times  \dfrac{e_{1} - e_{2}}{e_{1}}
\end{equation}
where $ e_{1} $ represents the error related to the reference method, and $e_2$ represents our approach's error.
\end{comment}












==> sec/exp_setup_v2_Tai.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{subsec:exp_setup}


\input{sec/datasets_v2_Aref}


\subheader{Baseline Detector Training}
We obtained the baseline detector by training MISLnet~\cite{mislnet} to distinguish between real and synthetic images on our baseline detector dataset. We chose MISLnet as the architecture for our experiments because it is lightweight and has been shown repeatedly to obtain strong performance on detecting synthetic images~\citethis. We trained MISLnet using a Cross-Entropy Loss function via the ADAM optimizer~\citethis with a constant learning rate of $5.0 \times 10^{-5}$. This model resulted in an accuracy of 0.95 and an area under the ROC curve (AUC) of 0.99 on the testing portion of our baseline detector dataset. Additionally, in Sec.~\ref{subsec:exp4_diff_arch} , we compared the performance of our approach and others using other baseline architectures, such as: ResNet-50~\cite{resnet}, SR-Net~\citethis, and DenseNet~\citethis.

\subheader{Expert Detector Training}
After we trained the baseline detector, we use this detector to create one expert detector for each new and emerging generators. 
To do this, each expert is fine-tuned on a small set of data, 
which is composed of fixed equal amounts of 
real images from the baseline detector dataset, 
and synthetic images from this dataset 
with additional images from the new generator. 
%
At every new generator's emergence, we trained the expert detector for a fixed (\TODO{X}) number of steps using the ADAM optimizer~\citethis with a constant learning rate of \TODO{X}. After fine-tuning, the network weights of these experts are frozen and never updated again.

\subheader{\reasoner Training}
After obtaining a new expert detector for an emerging synthetic image generator, we trained the \reasoner to combine the knowledge from all available experts. This training is done using a fixed small number of samples, 
which is composed of identical amounts of 
real images from the baseline detector dataset, 
and synthetic images that are
equally-distributed over all known generators.
%
At every new generator's emergence, we trained the expert detector for a fixed (\TODO{X}) number of steps using the ADAM optimizer~\citethis with a constant learning rate of \TODO{X}. 

\subheader{Size of Emerging Generator's Data}
As stated \hyperref[subhead:emerging_gen_dataset]{earlier} in this section, the amount of data, from any emerging generator, available for updating the baseline detector is 500 synthetic images, unless stated otherwise.

\subheader{Memory Buffer}
Throughout all experiments in this paper, we fixed memory buffer - the number of samples kept from previously known generators, including real images - at 1000 images (where 500 images are real and 500 images are synthetic). The synthetic images are then equally distributed among all previously known generators.


\subheader{Performance Metrics}
To evaluate the performance of our proposed approach and others, we chose the Area Under the ROC Curve (AUC) metric. 
% \TODO{Maybe say that we also present accuracy but in the supplemental??}
Additionally, to obtain a more complete picture of our performance, we provided the Relative Error Reduction metric with respect to the second best performing method, reported as a percentage. This metric is calculated such that
\skipless
\begin{equation}
	RER = 100 \times \frac{\text{AUC}_{N} - \text{AUC}_{R}}{1 - \text{AUC}_{R}}, 
\end{equation}
where $\text{AUC}_{R}$ is the AUC of the referencing method, and $\text{AUC}_{N}$ is the AUC of the method being compared against.

\skipnormal

\subheader{Competing Methods}
We compared our method against a total of 8 competing continual learning approaches.
These include a simple fine-tuning approach,
and 7 other state-of-the-art continual learning approaches, such as: 
1) Learning Without Forgetting (LWF)~\citethis, 
2) Experience Replay (ER)~\citethis, 
3) Dark Experience Replay (DER++)~\cite{der},
4) Unified Domain Incremental Learning (UDIL)~\cite{udil},
5) Incremental Classifier and Representation Learning (ICaRL)~\citethis,
6) Multi-Task Single-Classifier (MT-SC)~\citethis, and
7) Multi-Task Multi-Classifier (MT-MC)~\citethis, and
Note that we benchmarked all algorithms using code directly provided by respective authors with the exception of ICaRL in which we implemented the method ourselves.

==> sec/exp_setup_v3_Aref.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{subsec:exp_setup}


\input{sec/datasets_v2_Aref}


\subheader{Baseline Detector Training}
We obtained a baseline detector by training MISLnet~\cite{mislnet} to distinguish between real and synthetic images in our baseline detector dataset. We chose MISLnet as the architecture for our experiments because it is lightweight and has shown repeatedly to obtain strong performance on detecting synthetic images~\citethis. We trained MISLnet using a Cross-Entropy Loss function via the ADAM optimizer~\citethis with a constant learning rate of $5.0 \times 10^{-5}$. This model resulted in an accuracy of 0.97 and an area under the ROC curve (AUC) of 0.99 on the testing portion of our baseline detector dataset. Additionally, in Sec.~\ref{subsec:exp4_diff_arch}, we compared the performance of our approach and others using other baseline architectures, such as: ResNet-50~\cite{resnet}, SR-Net~\citethis, and DenseNet~\citethis.

\subheader{Expert Detector Training}
After we trained the baseline detector, we used this detector to create one expert embedder for each new emerging generator. 
At every new generator's emergence, the baseline detector is fine-tuned on a small set of data, which has a fixed size for all the new generators. This set is composed of equal amounts of 
synthetic images from the new generator and real images from the baseline dataset. After fine-tuning, the network weights of these experts are frozen and never updated again.

% After we trained the baseline detector, we use this detector to create one expert detector for each new and emerging generators. 
% To do this, each expert is fine-tuned on a small set of data, 
% which is composed of fixed equal amounts of 
% real images from the baseline detector dataset, 
% and synthetic images from this dataset 
% with additional images from the new generator. 

\subheader{\reasoner Training}
After obtaining a new expert embedder for an emerging synthetic image generator, we trained the \reasoner to combine the knowledge from all available experts. We minimized a binary cross-entropy loss function using the ADAM optimizer over a fixed small number of samples.
The training dataset at each step is composed of identical amounts of real images from the baseline detector dataset, 
and synthetic images that are
uniformly distributed over all known generators. 
% 


% After obtaining a new expert detector for an emerging synthetic image generator, we trained the \reasoner to combine the knowledge from all available experts. This training is done using a fixed small number of samples, 
% which is composed of identical amounts of 
% real images from the baseline detector dataset, 
% and synthetic images that are
% equally-distributed over all known generators.
% %
% At every new generator's emergence, we trained the expert detector for a fixed (\TODO{X}) number of steps using the ADAM optimizer~\citethis with a constant learning rate of \TODO{X}.



\subheader{Size of Emerging Generator's Data}
As stated \hyperref[subhead:emerging_gen_dataset]{earlier} in this section, the amount of available data for updating the baseline detector is 500 synthetic images for any emerging generator, unless stated otherwise.

\subheader{Memory Buffer}
Throughout all experiments in this paper, we fixed the size of memory buffer, $\mathcal{M}$, to 1000 images from which 500 are synthetic and 500 are real. The synthetic images are then equally distributed among all previously known generators.


\subheader{Performance Metrics}
To evaluate the performance of our proposed approach and others, we chose the Area Under the ROC Curve (AUC) metric. 
% \TODO{Maybe say that we also present accuracy but in the supplemental??}
Additionally, in order to obtain a more complete picture of our performance, we provided the Relative Error Reduction (RER) with respect to the second best performing method, reported as a percentage. This metric is calculated as follows:
\skipless
\begin{equation}
	RER = 100 \times \frac{\text{AUC}_{N} - \text{AUC}_{R}}{1 - \text{AUC}_{R}}, 
\end{equation}
where $\text{AUC}_{R}$ is the AUC of the referencing method, and $\text{AUC}_{N}$ is the AUC of the method being compared against.

\skipnormal

\subheader{Competing Methods}
We compared our method against a total of 8 competing continual learning approaches.
These include a simple fine-tuning approach,
as well as 7 other well-established and state-of-the-art continual learning approaches, such as: 
1) Learning Without Forgetting (LWF)~\citethis, 
2) Experience Replay (ER)~\citethis, 
3) Dark Experience Replay (DER++)~\cite{der},
4) Unified Domain Incremental Learning (UDIL)~\cite{udil},
5) Incremental Classifier and Representation Learning (ICaRL)~\cite{rebuffi2017icarl},
6) Multi-Task Single-Classifier (MT-SC)~\cite{marra2019incremental}, and
7) Multi-Task Multi-Classifier (MT-MC)~\cite{marra2019incremental}.
Note that we benchmarked LWF, ER, DER++, and UDIL algorithms using the code provided by \cite{udil}. Additionally we benchmarked ICaRL, MT-SC, and MT-MC using our own implementations.  

==> sec/exp_setup_v4_Tai.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{subsec:exp_setup}


\input{sec/datasets_v3_Manil}


\subheader{Baseline Detector Training}
We obtained a baseline detector by training MISLnet~\cite{mislnet} to distinguish between real and synthetic images in our baseline detector dataset. We chose MISLnet as the architecture for our experiments because it is lightweight and has shown repeatedly to obtain strong performance on detecting synthetic images~\cite{Bayar_2017_ICASSP, Bayar_2016_IHMMSEC, Mayer_2020_ICASSP, FSG, MISLgan}. We trained MISLnet using a Cross-Entropy Loss function via the ADAM optimizer~\cite{Adam} with a constant learning rate of $5.0 \times 10^{-5}$. This model resulted in an accuracy of 0.97 on the testing portion of our baseline detector dataset. 
%Additionally, in Sec.~\ref{subsec:exp4_diff_arch}, we compared the performance of our approach and others using other baseline architectures, such as: ResNet-50~\cite{resnet}, SR-Net~\citethis, and DenseNet~\citethis.

\subheader{Expert Detector Training}
The training procedure involved to create these experts are detailed in Sec.~\ref{subsec:new_expert_training}. We note that, after fine-tuning, the network weights of these experts are frozen and never updated again.


\subheader{\Reasoner Training}
We trained this network to combine the knowledge from all available experts using the procedure stated in Sec.~\ref{subsec:ekfn_training}.


\subheader{Size of New Generator's Data}
In the following experiments, the amount of available data from each new generator is 500 synthetic images, unless stated otherwise.

\subheader{Memory Buffer}
Throughout all experiments in this paper, we fixed the size of memory buffer, $\mathcal{M}$, to 1000 images from which 500 are synthetic and 500 are real. The synthetic images are then equally distributed among all previously known generators. We note that the memory buffer is continually updated after each step to include samples of the new generator.


\subheader{Performance Metrics}
To evaluate the performance of our proposed approach and others, we chose the Area Under the ROC Curve (AUC) metric. 
% \TODO{Maybe say that we also present accuracy but in the supplemental??}
Additionally, in order to obtain a more complete picture of our performance, we provided the Relative Error Reduction (RER) with respect to the second best performing method, reported as a percentage. This metric is calculated as follows:
\skipless
\begin{equation}
	RER = 100 \times \frac{\text{AUC}_{N} - \text{AUC}_{R}}{1 - \text{AUC}_{R}}, 
\end{equation}
where $\text{AUC}_{R}$ is the AUC of the referencing method, and $\text{AUC}_{N}$ is the AUC of the method being compared against.

\skipnormal

\subheader{Competing Methods}
We compared our method against multiple approaches. These include two naive approaches:
Baseline, where the baseline detector is never updated and Fine-tuning, where the baseline detector is updated only on data from the new generator. Along with these we also compared against seven well-established and state-of-the-art continual learning approaches: 
Learning Without Forgetting (LWF)~\cite{LWF}, 
Experience Replay (ER)~\cite{ER}, 
Dark Experience Replay (DER++)~\cite{der},
Unified Domain Incremental Learning (UDIL)~\cite{udil},
Incremental Classifier and Representation Learning (ICaRL)~\cite{rebuffi2017icarl},
Multi-Task Single-Classifier (MT-SC)~\cite{marra2019incremental}, and
Multi-Task Multi-Classifier (MT-MC)~\cite{marra2019incremental}.
Note that we benchmarked LWF, ER, DER++, and UDIL algorithms using the code provided by \cite{udil}. 

% Additionally we benchmarked ICaRL, MT-SC, and MT-MC using our own implementations.  

==> sec/experiments_v0.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
We ran a series of experiments to demonstrate our method's ability to adapt a baseline detector to be able to detect images from a new synthetic image generator. Basic experimental procedures are described below.

\subheader{Baseline Detectors Architectures} 
To train our baseline detectors we use two different architectures: ResNet50~\cite{resnet} which is widely used for synthetic image detection~\citethis, and MISLnet~\cite{mislnet} which is used for forensic manipulation detection~\citethis. These networks are trained on randomly sampled patches of size $256 \times 256$ obtained from the baseline training dataset. 
%
The ResNet50 is trained with an initial learning rate of $1.0 \times 10^{-4}$, which is further decayed by a factor of $0.75$ every 3 epochs. This model has an accuracy of $0.9593$ and an AUC of $0.9932$ on the baseline test dataset.
%
The MISLnet, on the other hand, is trained with a constant learning rate of $5.0 \times 10^{-5}$, and achieves an accuracy of $0.9732$ and an area under the ROC curve (AUC) of $0.9972$ on the test dataset.

\subheader{Baseline Detectors Testing Procedure}
To evaluate the baseline detectors performance, we used the test dataset described in Sec.~\ref{subsec:baseline_ds}, and report the accuracy and the AUC metrics. 

\subheader{Rotating Experiment Testing Procedure}
To test this scenario, we used the test sets described in Sec.~\ref{subsec:dataset_cl}. For each $G_i \in \mathbb{G}$, we evaluated the trained models performance on $D^N_{G_i}$ (the training dataset associated with $G_i$) and $D^N_{G_0}$ (the dataset associated with the GANs in the baseline dataset) in terms of accuracy and AUC. Then, we calculated the average of those metrics, which in total, yielded 20 average accuracies and 20 average AUCs. Finally, we separately report the mean of average accuracies and that of AUCs. We \textit{\textbf{can}} formalize those metrics as follows: ....


\subheader{Incremental Learning Experiment Testing Procedure}
In this setting, the incremental learner's goal is to reliably detect the data from the new generator as well as maintaining its performance on the previous data. Therefore, we evaluated our models performance by testing it against all of the $D^N_{G_i}$ (test datasets associated with $G_i$) for all $i \le t$, where $t$ indicates the index of the current episode. We denote the accuracy and the AUC of the model on $D^N_{G_j}$ after training on $D^N_{G_i}$ as $R_{i,j}$, and $S_{i,j}$, respectively.  Finally, we report the average of those metrics at the end of each episode $t$:
\begin{equation}
 \label{eq:avg_metrics}
 A_t = \frac{1}{t} \sum_{1}^{k} R_{t, k}, \: B_t = \frac{1}{t} \sum_{1}^{k} S_{t, k}
\end{equation}


\subheader{Competing Methods}
We compared our method against currently existing methods appropriate for our problem setting. First, we include a naive approach to address this problem, which is simply fine-tuning the baseline detectors on each upcoming sequence of data. Additionally, we include well-established and state-of-the-art continual learning methods, such as Experience Replay (ER)~\citethis, Dark Experience Replay (DER)~\citethis, and Unified Domain Incremental Learning (UDIL)~\citethis.
One could also solely depend on transferability of the baseline detectors; therefore, we include the baseline detectors performance as a reference.

\subsection{Experiment \#1}
\begin{itemize}
	\item why?
\end{itemize}
\subsection{Experiment \#2}
\begin{itemize}
	\item why?
\end{itemize}
\subsection{Experiment \#3}
\begin{itemize}
	\item why?
\end{itemize}

==> sec/guidelines/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/guidelines/1_intro_guideline.tex <==
\section{Introduction}
%\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/guidelines/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/guidelines/2_formatting_guide.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/guidelines/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/guidelines/3_finalcopy_guide.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/guidelines/X_suppl_guide.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary


\section{Rationale}
\label{sec:rationale}
% 
Having the supplementary compiled together with the main paper means that:
% 
\begin{itemize}
\item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
\item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
\item When submitted to arXiv, the supplementary will already included at the end of the paper.
\end{itemize}
% 
To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.

==> sec/intro_v0.tex <==
\section{Introduction}
\label{sec:introduction}

\textbf{THIS IS A PLACEHOLDER INTRO}

Over the past several years, a number of AI-based techniques have been developed to create visually realistic synthetic images.  
%
While these synthetic image generators can be used for creative or artistic purposes, they can also be used to malicious ones.  Specifically, they enable the creation of fake images that can be used for misinformation or disinformation.

In response to this, researchers have developed a number of techniques to detect synthetic images.  Prior work has shown that image generators leave behind unique traces in synthetic images~\cite{ }.  Forensic neural networks can be trained to learn these traces and use them to accurately detect synthetic images from a wide variety of generators~\cite{ }.

Despite this, forensics research has also shown that synthetic image detectors can experience difficulty detecting images from generators whose traces are significantly different from generators seen during training.  For example, Corvi et al. showed that detectors trained using only GAN generated images achieve low performance when confronted with images made using diffusion models~\cite{ }.  At the same time, rapid advancements in AI have led to the continual development of new generation techniques that potentially leave significantly different traces than existing generators.  

As a result, synthetic image generators must be continually updated to detect images from new generators.

Additional points to make:
\begin{itemize}
\item Challenges posed by updating
    \begin{enumerate}
    \item catastrophic forgetting
    \item don't want to have to store and continually retrain large dataset
    \end{enumerate}
\item Also, we often will have limited data from a newly emerging generator, particularly if generator is not yet publicly available (i.e. sora)
\item need techniques to update generator
\item Continual learning approaches are useful, but they have drawbacks: try to update network so that this one network can learn traces from all generators (previously seen generator as well as new generator)
\item In this paper, we propose a new approach for continually updating synthetic image detectors.
    \begin{enumerate}  
    \item Instead of using one network to capture all forensic traces, we create an ensemble of expert embedders
    \item each embedder created through transfer learning and is able to accurately capture trace from a specific generator
    \item the resulting sequence of embeddings is then analyzed by an Expert Knowledge Fusion Network that uses info from all experts to accurately perform detection
    \item both expert embedder and EKFN can be trained using limited amount of data
    \end{enumerate}
\item We present results showing that E3 can signifcantly outperform competing continual learning approaches, including those specifically designed to update synthetic image detectors

\item The novel contributions of this paper are:
    \begin{enumerate}
        \item LIST THESE HERE (previously written on whiteboard)
    \end{enumerate}

\end{itemize}









==> sec/intro_v1_MCS.tex <==
% intro_v1_MCS

\section{Introduction}
\textbf{[MADE W/ CHATGPT USING MATT'S NOTES.  NEEDS REVISION]}

In recent years, the proliferation of AI-driven technologies has led to the development of sophisticated techniques for generating synthetic images with striking visual realism. While these advancements have paved the way for various creative applications, they have also raised concerns regarding their potential misuse for malicious purposes, such as the creation of deceptive or misleading content.
\input{figures/front_page_graphics}
To address these challenges, considerable research efforts have been directed towards the development of synthetic image detection techniques. Prior work has demonstrated the effectiveness of forensic neural networks in discerning synthetic images by identifying unique traces left behind by different image generators. However, a significant limitation of existing detectors arises when they encounter images generated by previously unseen or emerging techniques, whose traces differ substantially from those in the training data.

This poses a critical need for continually updating synthetic image detectors to adapt to new generators. However, this task presents several challenges. Traditional approaches to updating detectors often encounter issues such as catastrophic forgetting and the impracticality of storing and retraining on large datasets~\citethis. Moreover, limited data availability from newly emerging generators, especially those not yet publicly accessible, further complicates the updating process.

In this paper, we propose a novel approach to address these challenges. Instead of relying on a single network to capture all forensic traces, we introduce an Ensemble of Expert Embedders (E3) framework. Each expert embedder is created through transfer learning and specializes in capturing traces from a specific image generator. These expert embedders collectively generate a sequence of embeddings, which are then analyzed by an Expert Knowledge Fusion Network (EKFN). The EKFN leverages information from all expert embedders to accurately perform synthetic image detection, even with limited data availability.

Our experimental results demonstrate that the proposed E3 framework significantly outperforms existing continual learning approaches, including those tailored specifically for updating synthetic image detectors. The key contributions of this paper include the development of the E3 framework, which offers an effective solution for adapting synthetic image detectors to new generators while mitigating the challenges associated with limited data and catastrophic forgetting. 


==> sec/old_and_temp_files/method_v0.tex <==
\section{Proposed Method}

\red{\textbf{Work in Progress}}

\subsection{Motivation}

Assume $f(i)$ is a synthetic image detector. $f$ can be decomposed into two conceptual parts $\varphi$ and $h$, where $\varphi : \mathcal{I}~\rightarrow~\mathcal{X}$ is a network that captures forensic traces of the input and outputs an embedding, and $h(\cdot)$ is a classifier that maps the embedding to a detection decision, $\delta$. Consider a set of synthetic image detectors $\{f_0, f_1, f_2, \ldots\}$, we write $f_l = h_l \circ \varphi_l$ and denote $\ubar{x}{l} = \varphi_l(i)$, where $\ubar{x}{l} \in \mathcal{X}_l$ is the embedding resulted from applying the embedder $\varphi_l$ on image $i$ and $l \in \mathbb{Z}$ is an arbitrary integer.

Let $f_0 = h_0 \circ \varphi_0$ be a baseline synthetic image detector with embedding space $\mathcal{X}_0$ which is trained on a large dataset, $\mathcal{B}$. We refer to the set of generators used to make the synthetic images in $\mathcal{B}$ as $\mathcal{G}^{(0)}$. Now, consider a new generator $g_k \notin \mathcal{G}^{(0)}$ emerges. We need to find $f_k$ to detect images made by $g_l$ without forgetting how to detect those synthesized by generators in $\mathcal{G}^{(0)}$.

Continual learning tries to update the entire network $f_0$, effectively trying to learn a new embedding space $\mathcal{X}'$ that captures traces from $g_k$ as well as generators in $\mathcal{G}^{(0)}$. Since traces from these generators may be very different, learning $\mathcal{X}'$ can become an increasingly challenging task particularly with limited amounts of data being available from each generator.

To overcome this, we propose a new Ensemble of Expert Embedders (EEE) approach. After the introduction of $g_k$, instead of using only a single embedding space to capture forensic traces of all generators, we learn a new embedding space, $\mathcal{X}_k$, and use the set of already learned embedding spaces, $\{\mathcal{X}_0, \dots, \mathcal{X}_k\}$. We incrementally learn the set of embedding spaces by sequentially training a set of expert embedders $\mathcal{E}_k = \{\varphi_0, \ldots, \varphi_k\}$ as each new generator emerges. Each $\varphi_{l \ne k} \in \mathcal{E}_k$ specifically learns to capture forensic traces left by the generation process of $g_l$. However, it might not necessarily capture the traces associated with generators other than $g_k$.
% 

Subsequently, we analyze the sequence of embeddings from these experts using a reasoner (\textbf{\red{?}}) network trained with a limited data budget to produce a single detection decision. This network utilizes a transformer based self-attention mechanism to identify evidence from key experts in order to reliably make an accurate decision.


\subsection{Problem Setup}
Assume baseline detector $f_0$ has been trained to detect images generated by a set of generators $\mathcal{G}_0$ using a large baseline training dataset $\mathcal{B}$. Assume $\mathcal{B}$ is so large that we do not wish to retain it or to use it for training every time a new synthetic image generator emerges. 
%
To address this, we create a memory dataset $\mathcal{M}_0$ of $2N_1$ images, where $N_1 \ll |\mathcal{B}|$. Specifically, $\mathcal{M}_0$ is consisted of a set $\mathcal{R}$ of $N_1$ real images and a set $\mathcal{S}_0$ of $N_1$ synthetic images from generators in $\mathcal{G}_0$. This dataset will be updated to $\mathcal{M}_k$ as the $k$-th generator, $g_k$, emerges but will always be limited to a fixed number of images \emph{s.t.} $|\mathcal{M}_k|=2N_1$.
%
Additionally, we assume that we are able to collect $N_2$ images from $g_k$ to form dataset $\mathcal{D}_k$. We also assume the only data available to update the detector at the emergence of $g_k$ is $\mathcal{M}_k \cup \mathcal{D}_k$. For the rest of the paper, we will refer to the process of updating a synthetic image detector as one \emph{episode}.

\subsection{Training New Expert Embedder}
When a new synthetic image generator $g_{k > 0}$ emerges we need to make a new expert to capture traces associated with it. To do this, we utilize $\mathcal{D}_k$ and $\mathcal{R}$ to train an expert embeddor $\varphi_k$ through transfer learning.
%
Specifically, we fine-tune $f_0$ using $\mathcal{D}_k \cup \mathcal{R}$ to get an intermediate expert detector $\hat{f}_k$. This new detector will likely experience catastrophic forgetting and lose significant ability to detect generators other than $g_k$. Then, we extract expert embedder $\varphi_k$ by discarding the classification component $h_k$ of $\hat{f}_k$. This procedure is outlined in Alg.~\ref{alg:ft}. 

%After obtaining the expert embedder $\varphi_k$, we update $\mathcal{M}_{k-1}$ to $\mathcal{M}_{k}$, which will be used as the only training data for the classification sub-network. Additionally, we form $\mathcal{G}_k = \mathcal{G}_{k-1} \cup \{g_k\}$. (\red{we need to put these last two steps in the main algorithm probably}).

\subsection{History Management}
After training the expert $\varphi_k$, we need to update the set of already existing expert embedders. Furthermore, we need to update the memory with the recently observed synthetic data, $\mathcal{D}_k$ so that the future generations of the detector can still detect images from $g_k$.
We employ a uniform random sampling strategy to have a balanced set of synthetic image data from each generator in the memory. We also add $g_k$ to the set of previously observed generators. The details is provided in Alg.~\ref{alg:mem}

\begin{algorithm}
	\caption{Update History}\label{alg:mem}
	\begin{algorithmic}[1]
		\Procedure{UpdateHistory}{$\varphi_k, g_k, \mathcal{D}_k,\mathcal{S}_{k-1}, \mathcal{R}$}
		\State $\mathcal{E}_k \gets \mathcal{E}_k \cup \{\varphi_k\}$
		\State $\mathcal{G}^{(k)} \gets \mathcal{G}^{(k-1)} \cup \{g_k\}$
		\State $\mathcal{M}_{k} \gets \{\}$
		\For{$l \in \{0, \ldots, k\}$}
			\State Let $\mathcal{S}$ be a random subset of $D_l$ with size $N_1(\frac{k-1}{k})$
			\State $\mathcal{M}_{k} \gets \mathcal{M}_{k} \cup \mathcal{S}$
		\EndFor
		\State $\mathcal{M}_{k} \gets \mathcal{M}_{k} \cup \mathcal{R}$
		\State \Return $\mathcal{M}_{k}, \mathcal{G}^{(k)}, \mathcal{E}_k$
		\EndProcedure
		
		
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{\:\: Train $\varphi_k$}\label{alg:ft}
	\begin{algorithmic}[1]
		\Procedure{TrainExpert}{$f_0, \mathcal{D}_k, \mathcal{R}, \mathcal{P}$}
		\State Form $\mathcal{T} = \mathcal{D}_k \cup \mathcal{R}$
		\State Fine-tune $f_0$ with $\mathcal{T}$ to get $\hat{f}_k$ using $\mathcal{P}$
		\State Extract $\varphi_k$ by discarding $h_k$ of $\hat{f}_0$
		\State \Return $\varphi_k$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\subsection{Training Reasoner}
After training the expert embedder $\varphi_k$, we train a reasoner (\red{?}) network, $\psi_k$, to perform classification. This network needs to make a decision based on the sequence of embeddings produced by embedders in $\mathcal{E}_k$, which we define as $\mathcal{L}_k = \{\ubar{x}{l} \: | \: \varphi_l \in \mathcal{E}_k \}$.
%
The network analyzes $\mathcal{L}_k$, using a transformer to treat each input embedding as a token in a sequence of forensic evidence. The transformer's output associated with $\ubar{x}{l}$, which we refer to as $\ubar{z}{l}$, contains information about the relevance of $\ubar{x}{l}$  with respect to itself and other embeddings in $\mathcal{L}_k$. We use $\psi$ as an attention mechanism to scale $\ubar{x}{l}$ by $\ubar{z}{l}$ and then provide the sequence of weighted embeddings to a classifier network composed of only a few linear layers. The training procedure of the reasoner is provided in Alg.~\ref{alg:reason}.

\begin{algorithm}
	\caption{\:\: Train $\psi_k$}\label{alg:reason}
	\begin{algorithmic}[1]
		\Procedure{TrainReasoner}{$\mathcal{M}_{k-1}, \mathcal{D}_{k},  \mathcal{E}_{k}, \varphi_k, \mathcal{P}$}
		\State $\mathcal{E}_{k} \gets \mathcal{E}_{k-1} \cup \{\varphi_k\}$
		
		\State Form $\mathcal{M}_{k}$ by updating $\mathcal{M}_{k-1}$ with $\mathcal{S}_{k-1}, \mathcal{R}, \mathcal{D}_{k}$
		
		\For{$i \in  \mathcal{M}_{k}$}
			\State $\mathcal{L}_k^i \gets \{\ubar{x}{l} \: | \: \varphi_l \in \mathcal{E}_k \}$
			\State Feed $\mathcal{L}_k^i$ to the transformer to get $\ubar{z}{l}$s
			\State Scale $\mathcal{L}_k^i$ by $\ubar{z}{l}$s
			\State Calculate Loss
			\State Backprop
			
      	\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


\subsection{Summary}
To sum up, we perform the following steps in order to produce a synthetic image detector $f_k$ after emerging $g_k$. First, we fine-tune the baseline detector $f_0$ with a small amount of data generated by $g_k$ to create $\varphi_k$. After that, we add $\varphi_k$ to the set of existing expert embedders to form $\mathcal{E}_k$. Then, we employ $\mathcal{E}_k$ to generate a sequence of embeddings for each data point in $\mathcal{M}_k$.

\begin{algorithm}
	\caption{\:\: Train $f_k$}\label{alg:get_fk}
	\begin{algorithmic}[1]
		\Procedure{$\tau_3$}{$f_0, \mathcal{D}_k, \mathcal{R}, \mathcal{P}$}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

%\begin{enumerate}
%	\item  Fine-tune the baseline detector $f_0$ with a small amount of data generated by $g_k$ to create $\varphi_k$.~(\ref{alg:ft})
%	\item Add $\varphi_k$ to the set of existing expert embedders to form $\mathcal{E}_k$.
%	\item Employ $\mathcal{E}_k$ to generate a sequence of embeddings $\mathcal{L}_k$ for each image in $\mathcal{M}$
%	\item Update the weights of $\psi_k$ to minimize a binary cross-entropy loss
%	\item Repeat 3 until done
%\end{enumerate}





















==> sec/old_and_temp_files/method_v1.tex <==
\section{Proposed Method}

\red{\textbf{Work in Progress}}

%\subsection{Motivation}
%
%Assume $f(i)$ is a synthetic image detector. $f$ can be decomposed into two conceptual parts $\varphi$ and $h$, where $\varphi : \mathcal{I}~\rightarrow~\mathcal{X}$ is a network that captures forensic traces of the input and outputs an embedding, and $h(\cdot)$ is a classifier that maps the embedding to a detection decision, $\delta$. Consider a set of synthetic image detectors $\{f_0, f_1, f_2, \ldots\}$, we write $f_l = h_l \circ \varphi_l$ and denote $\ubar{x}{l} = \varphi_l(i)$, where $\ubar{x}{l} \in \mathcal{X}_l$ is the embedding resulted from applying the embedder $\varphi_l$ on image $i$ and $l \in \mathbb{Z}$ is an arbitrary integer.
%
%Let $f_0 = h_0 \circ \varphi_0$ be a baseline synthetic image detector with embedding space $\mathcal{X}_0$ which is trained on a large dataset, $\mathcal{B}$. We refer to the set of generators used to make the synthetic images in $\mathcal{B}$ as $\mathcal{G}^{(0)}$. Now, consider a new generator $g_k \notin \mathcal{G}^{(0)}$ emerges. We need to find $f_k$ to detect images made by $g_l$ without forgetting how to detect those synthesized by generators in $\mathcal{G}^{(0)}$.
%
%Continual learning tries to update the entire network $f_0$, effectively trying to learn a new embedding space $\mathcal{X}'$ that captures traces from $g_k$ as well as generators in $\mathcal{G}^{(0)}$. Since traces from these generators may be very different, learning $\mathcal{X}'$ can become an increasingly challenging task particularly with limited amounts of data being available from each generator.
%
%To overcome this, we propose a new Ensemble of Expert Embedders (EEE) approach. After the introduction of $g_k$, instead of using only a single embedding space to capture forensic traces of all generators, we learn a new embedding space, $\mathcal{X}_k$, and use the set of already learned embedding spaces, $\{\mathcal{X}_0, \dots, \mathcal{X}_k\}$. We incrementally learn the set of embedding spaces by sequentially training a set of expert embedders $\mathcal{E}_k = \{\varphi_0, \ldots, \varphi_k\}$ as each new generator emerges. Each $\varphi_{l \ne k} \in \mathcal{E}_k$ specifically learns to capture forensic traces left by the generation process of $g_l$. However, it might not necessarily capture the traces associated with generators other than $g_k$.
%% 
%
%Subsequently, we analyze the sequence of embeddings from these experts using a reasoner (\textbf{\red{?}}) network trained with a limited data budget to produce a single detection decision. This network utilizes a transformer based self-attention mechanism to identify evidence from key experts in order to reliably make an accurate decision.

\subsection{Overview}
Assume we a have synthetic image detector trained on a large dataset of real and GAN-generated images, \textit{a.k.a} baseline detector. This detector is capable of identifying images generated by the GANs available during training. However, as previous research has shown, this detector will not be able to accurately detect images from new generators whose data were not present in the baseline detector training dataset~\cite{luisa-diff}. This problem is highlighted when new families of generators emerge as the forensic traces they leave behind could be significantly different compared to other families. For example, a synthetic image detector trained on images generated by GANs has a poor performance on the images generated by diffusion models~\cite{luisa-diff}. 
%

To reliably detect images from the new generators we need to update the baseline detector. A naive approach is to fine-tune the baseline detector with data from the new generator, but this will lead to significant catastrophic forgetting. Another approach is to re-train the baseline detector from scratch, which requires a large amount of data from the new generator to result in a high overall performance. Re-training becomes increasingly more problematic as new synthetic image and \emph{video} generators capable of generating super-realistic media emerge rapidly. Storing a large dataset that grows every time a new generator emerges can be expensive. Furthermore, access to the new generator can possibly be limited; therefore, it might be impossible to gather large amounts of data from it. 

Another family of methods that could be employed to update the baseline detector is continual learning. Continual learning tries to update the entire baseline network, effectively trying to learn a new embedding space that captures traces from the new generator as well as generators available during training the baseline detector. Since traces from these generators may be very different, learning the embedding space can become an increasingly challenging task, particularly with limited amounts of data being available from each generator.

To overcome the limitations of the previous work, we propose a new \mixture approach. After the introduction of each new generator, unlike continual learning, we learn a new embedding space to specifically capture the forensic traces of only the new generator. As each new generator emerges, we incrementally train a set of expert embedders. Each of these expert embedders can dependably detect the images synthesized from its associated generator. However, it might not be able to detect images from other generators due to catastrophic forgetting. To make the final detection decision, we further fuse the representations created by the set of expert embedders via a network called \reasoner.

\subsection{Problem Setup}
Assume baseline detector $f_0$ has been trained to detect images generated by a set of generators $\mathcal{G}_0$ using a large baseline training dataset $\mathcal{B}$. Assume $\mathcal{B}$ is so large that we do not wish to retain it or to use it for training every time a new synthetic image generator emerges. 
%
To address this, we create a memory dataset $\mathcal{M}_0$ of $2N_1$ images, where $N_1 \ll |\mathcal{B}|$. Specifically, $\mathcal{M}_0$ is consisted of a set $\mathcal{R}$ of $N_1$ real images and a set $\mathcal{S}_0$ of $N_1$ synthetic images from generators in $\mathcal{G}_0$. This dataset will be updated to $\mathcal{M}_k$ as the $k$-th generator, $g_k$, emerges but will always be limited to a fixed number of images \emph{s.t.} $|\mathcal{M}_k|=2N_1$.
%
Additionally, we assume that we are able to collect $N_2$ images from $g_k$ to form dataset $\mathcal{D}_k$. We also assume the only data available to update the detector at the emergence of $g_k$ is $\mathcal{M}_k \cup \mathcal{D}_k$. For the rest of the paper, we will refer to the process of updating a synthetic image detector as one \emph{episode}.

\subsection{Training New Expert Embedder}
When a new synthetic image generator $g_{k > 0}$ emerges we need to make a new expert to capture traces associated with it. To do this, we utilize $\mathcal{D}_k$ and $\mathcal{R}$ to train an expert embeddor $\varphi_k$ through transfer learning.
%
Specifically, we fine-tune $f_0$ using $\mathcal{D}_k \cup \mathcal{R}$ to get an intermediate expert detector $\hat{f}_k$. This new detector will likely experience catastrophic forgetting and lose significant ability to detect generators other than $g_k$. Then, we extract expert embedder $\varphi_k$ by discarding the classification component $h_k$ of $\hat{f}_k$. This procedure is outlined in Alg.~\ref{alg:ft}. 

%After obtaining the expert embedder $\varphi_k$, we update $\mathcal{M}_{k-1}$ to $\mathcal{M}_{k}$, which will be used as the only training data for the classification sub-network. Additionally, we form $\mathcal{G}_k = \mathcal{G}_{k-1} \cup \{g_k\}$. (\red{we need to put these last two steps in the main algorithm probably}).

\begin{algorithm}
	\caption{\:\: Train $\varphi_k$}\label{alg:ft}
	\begin{algorithmic}[1]
		\Procedure{TrainExpert}{$f_0, \mathcal{D}_k, \mathcal{R}, \mathcal{P}$}
		\State Form $\mathcal{T} = \mathcal{D}_k \cup \mathcal{R}$
		\State Fine-tune $f_0$ with $\mathcal{T}$ to get $\hat{f}_k$ using $\mathcal{P}$
		\State Extract $\varphi_k$ by discarding $h_k$ of $\hat{f}_0$
		\State \Return $\varphi_k$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\subsection{Training Reasoner}
After training the expert embedder $\varphi_k$, we train a reasoner (\red{?}) network, $\psi_k$, to perform classification. This network needs to make a decision based on the sequence of embeddings produced by embedders in $\mathcal{E}_k$, which we define as $\mathcal{L}_k = \{\ubar{x}{l} \: | \: \varphi_l \in \mathcal{E}_k \}$.
%
The network analyzes $\mathcal{L}_k$, using a transformer to treat each input embedding as a token in a sequence of forensic evidence. The transformer's output associated with $\ubar{x}{l}$, which we refer to as $\ubar{z}{l}$, contains information about the relevance of $\ubar{x}{l}$  with respect to itself and other embeddings in $\mathcal{L}_k$. We use $\psi$ as an attention mechanism to scale $\ubar{x}{l}$ by $\ubar{z}{l}$ and then provide the sequence of weighted embeddings to a classifier network composed of only a few linear layers. The training procedure of the reasoner is provided in Alg.~\ref{alg:reason}.

\begin{algorithm}
	\caption{\:\: Train $\psi_k$}\label{alg:reason}
	\begin{algorithmic}[1]
		\Procedure{TrainReasoner}{$\mathcal{M}_{k-1}, \mathcal{D}_{k},  \mathcal{E}_{k}, \varphi_k, \mathcal{P}$}
		\State $\mathcal{E}_{k} \gets \mathcal{E}_{k-1} \cup \{\varphi_k\}$
		
		\State Form $\mathcal{M}_{k}$ by updating $\mathcal{M}_{k-1}$ with $\mathcal{S}_{k-1}, \mathcal{R}, \mathcal{D}_{k}$
		
		\For{$i \in  \mathcal{M}_{k}$}
			\State $\mathcal{L}_k^i \gets \{\ubar{x}{l} \: | \: \varphi_l \in \mathcal{E}_k \}$
			\State Feed $\mathcal{L}_k^i$ to the transformer to get $\ubar{z}{l}$s
			\State Scale $\mathcal{L}_k^i$ by $\ubar{z}{l}$s
			\State Calculate Loss
			\State Backprop
			
      	\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


\subsection{Summary}
To sum up, we perform the following steps in order to produce a synthetic image detector $f_k$ after emerging $g_k$. First, we fine-tune the baseline detector $f_0$ with a small amount of data generated by $g_k$ to create $\varphi_k$. After that, we add $\varphi_k$ to the set of existing expert embedders to form $\mathcal{E}_k$. Then, we employ $\mathcal{E}_k$ to generate a sequence of embeddings for each data point in $\mathcal{M}_k$.

\begin{algorithm}
	\caption{\:\: Train $f_k$}\label{alg:get_fk}
	\begin{algorithmic}[1]
		\Procedure{$\tau_3$}{$f_0, \mathcal{D}_k, \mathcal{R}, \mathcal{P}$}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

%\begin{enumerate}
%	\item  Fine-tune the baseline detector $f_0$ with a small amount of data generated by $g_k$ to create $\varphi_k$.~(\ref{alg:ft})
%	\item Add $\varphi_k$ to the set of existing expert embedders to form $\mathcal{E}_k$.
%	\item Employ $\mathcal{E}_k$ to generate a sequence of embeddings $\mathcal{L}_k$ for each image in $\mathcal{M}$
%	\item Update the weights of $\psi_k$ to minimize a binary cross-entropy loss
%	\item Repeat 3 until done
%\end{enumerate}





















==> sec/suppl_v0.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary


\section{Rationale}
\label{sec:rationale}
% 
Having the supplementary compiled together with the main paper means that:
% 
\begin{itemize}
\item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
\item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
\item When submitted to arXiv, the supplementary will already included at the end of the paper.
\end{itemize}
% 
To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.

==> tables/exp1.tex <==
\begin{table*}
	\centering
	\caption{\label{tab:exp1} exp 1}
	\resizebox{0.95\linewidth}{!}{
		\begin{tblr}{
				width = 1.0\linewidth,
				colspec = {|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|[2pt]c|c|},
				column{1} = {l},
				vline{1-22} = {-}{},
				hline{1-2,12} = {-}{},
			}
			Method    & SD1.4 & GLD  & MJ   & DLM  & TT   & SD2.1 & CIP  & BG   & VQD  & DiG  & SG3  & GF   & DL2  & LD   & EG3  & PG   & SD1  & DDG  & DDP  & Avg. \\
			Baseline  & 0.89  & 0.98 & 0.85 & 0.86 & 0.81 & 0.89  & 0.76 & 0.77 & 0.85 & 0.76 & 0.98 & 0.73 & 0.97 & 0.81 & 0.98 & 0.89 & 0.87 & 0.67 & 0.78 & 0.85 \\
			Fine-Tune & 0.65  & 0.83 & 0.65 & 0.67 & 0.64 & 0.69  & 0.85 & 0.75 & 0.88 & 0.88 & 0.90 & 0.92 & 0.79 & 0.68 & 0.89 & 0.76 & 0.74 & 0.87 & 0.84 & 0.78 \\
			LWF       & 0.91  & 0.98 & 0.92 & 0.82 & 0.85 & 0.92  & 0.85 & 0.88 & 0.96 & 0.94 & 0.99 & 0.95 & 0.94 & 0.72 & 0.97 & 0.92 & 0.91 & 0.95 & 0.94 & 0.91 \\
			ER        & 0.94  & 0.99 & 0.97 & 0.96 & 0.96 & 0.94  & 0.99 & 0.91 & 0.98 & 0.98 & 0.99 & 0.99 & 0.99 & 0.90 & 1.00 & 0.96 & 0.94 & 0.99 & 0.99 & 0.97 \\
			DER++     & 0.94  & 0.99 & 0.96 & 0.95 & 0.95 & 0.93  & 0.98 & 0.89 & 0.97 & 0.97 & 0.99 & 0.98 & 0.99 & 0.90 & 1.00 & 0.96 & 0.93 & 0.99 & 0.98 & 0.96 \\
			UDIL      & 0.94  & 1.00 & 0.97 & 0.97 & 0.96 & 0.94  & 0.99 & 0.92 & 0.98 & 0.98 & 0.99 & 0.99 & 0.99 & 0.91 & 1.00 & 0.97 & 0.93 & 0.99 & 0.99 & 0.97 \\
			ICaRL     & 0.88  & 0.96 & 0.91 & 0.91 & 0.89 & 0.91  & 0.96 & 0.87 & 0.94 & 0.95 & 0.91 & 0.95 & 0.95 & 0.86 & 0.97 & 0.89 & 0.88 & 0.93 & 0.96 & 0.92 \\
			MT-SC      & 0.91  & 0.99 & 0.93 & 0.93 & 0.92 & 0.92  & 0.98 & 0.90 & 0.96 & 0.96 & 0.97 & 0.98 & 0.97 & 0.88 & 0.99 & 0.94 & 0.91 & 0.98 & 0.98 & 0.95 \\
			MT-MC      & 0.92  & 1.00 & 0.95 & 0.95 & 0.94 & 0.93  & 0.99 & 0.90 & 0.98 & 0.98 & 0.99 & 0.99 & 0.99 & 0.88 & 0.99 & 0.96 & 0.92 & 0.99 & 0.99 & 0.96 \\
			Ours      & 0.99  & 1.00 & 0.99 & 0.99 & 0.98 & 0.98  & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 & 1.00 & 0.96 & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.99 
		\end{tblr}
	}
\end{table*}

==> tables/exp2.tex <==
\begin{table*}
	\centering
	\caption{\label{tab:exp2} exp 2}
	\resizebox{0.95\linewidth}{!}{
		\begin{tblr}{
				width = 1.0\linewidth,
				colspec = {|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|},
				column{1} = {l},
				vline{1-21} = {-}{},
				vline{2} = {-}{},
				hline{1-2,12} = {-}{},
			}
			Method & SD1.4 & GLD & MJ & DLM & TT & SD2.1 & CIP & BG & VQD & DiG & SG3 & GF & DL2 & LD & EG3 & PG & SD1 & DDG & DDP\\
			Baseline & 0.89 & 0.91 & 0.86 & 0.83 & 0.80 & 0.79 & 0.76 & 0.73 & 0.73 & 0.71 & 0.73 & 0.71 & 0.73 & 0.72 & 0.74 & 0.74 & 0.74 & 0.72 & 0.71\\
			Fine-Tune & 0.65 & 0.79 & 0.73 & 0.81 & 0.83 & 0.83 & 0.80 & 0.84 & 0.82 & 0.82 & 0.85 & 0.85 & 0.73 & 0.79 & 0.81 & 0.70 & 0.76 & 0.83 & 0.74\\
			LWF & 0.90 & 0.91 & 0.89 & 0.89 & 0.88 & 0.89 & 0.86 & 0.85 & 0.85 & 0.85 & 0.82 & 0.82 & 0.72 & 0.80 & 0.82 & 0.81 & 0.80 & 0.83 & 0.79\\
			ER & 0.94 & 0.96 & 0.96 & 0.96 & 0.95 & 0.95 & 0.95 & 0.91 & 0.93 & 0.93 & 0.94 & 0.94 & 0.93 & 0.91 & 0.93 & 0.90 & 0.90 & 0.93 & 0.93\\
			DER++ & 0.96 & 0.96 & 0.92 & 0.91 & 0.88 & 0.89 & 0.86 & 0.84 & 0.83 & 0.82 & 0.82 & 0.82 & 0.79 & 0.81 & 0.82 & 0.82 & 0.82 & 0.82 & 0.80\\
			UDIL & 0.95 & 0.97 & 0.96 & 0.96 & 0.96 & 0.95 & 0.96 & 0.93 & 0.94 & 0.94 & 0.94 & 0.94 & 0.94 & 0.93 & 0.94 & 0.92 & 0.92 & 0.93 & 0.93\\
			ICaRL & 0.91 & 0.93 & 0.92 & 0.91 & 0.90 & 0.92 & 0.91 & 0.89 & 0.90 & 0.91 & 0.90 & 0.91 & 0.91 & 0.87 & 0.90 & 0.89 & 0.90 & 0.90 & 0.90\\
			MT-SC & 0.87 & 0.85 & 0.77 & 0.76 & 0.75 & 0.74 & 0.76 & 0.69 & 0.73 & 0.74 & 0.74 & 0.73 & 0.74 & 0.70 & 0.69 & 0.70 & 0.70 & 0.76 & 0.74\\
			MT-MC & 0.92 & 0.96 & 0.94 & 0.94 & 0.93 & 0.91 & 0.92 & 0.88 & 0.89 & 0.90 & 0.91 & 0.92 & 0.91 & 0.86 & 0.90 & 0.87 & 0.87 & 0.91 & 0.90\\
			Ours & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \textbf{0.98} & \textbf{0.98} & \textbf{0.98} & \textbf{0.98} & \textbf{0.98} & \textbf{0.97} & \textbf{0.97} & \textbf{0.97} & \textbf{0.97} & \textbf{0.97} & \textbf{0.97} & \textbf{0.97} & \textbf{0.97} & \textbf{0.97}
		\end{tblr}
	}
\end{table*}
